Early r-process Enrichment and Hierarchical Assembly Across the Sagittarius Dwarf Galaxy

Dwarf galaxies like Sagittarius (Sgr) provide a unique window into the early stages of galactic chemical evolution, particularly through their metal-poor stars. By studying the chemical abundances of stars in the Sgr core and tidal streams, we can gain insights into the assembly history of this galaxy and its early heavy element nucleosynthesis processes. We efficiently selected extremely metal-poor candidates in the core and streams for high-resolution spectroscopic analysis using metallicity-sensitive photometry from SkyMapper DR2, and Gaia DR3 XP spectra and proper motions. This allowed us to obtain a high-purity selection of Sgr members based on stellar kinematics while reducing the chances of potential contamination from the Milky Way halo. We present a sample of 37 Sgr stars with detailed chemical abundances, of which we identify 10 extremely metal-poor (EMP; $\rm{[Fe/H]} \le -3.0$) stars, 25 very metal-poor (VMP; $\rm{[Fe/H]} \le -2.0$) stars, and 2 metal-poor (MP; $\rm{[Fe/H]} \le -1.0$) stars. This sample increases the number of extremely metal-poor Sgr stars analyzed with high-resolution spectroscopy by a factor of five. Of these stars, 15 are identified as members of the Sgr tidal stream, while the remaining 22 are associated with the core. We derive abundances for up to 20 elements and identify no statistically significant differences between the element abundance patterns across the core and stream samples. Intriguingly, we identify stars that may have formed in ultra-faint dwarf galaxies that accreted onto Sgr, in addition to patterns of C and r-process elements distinct from the Milky Way halo. Over half of the sample shows a neutron-capture element abundance pattern consistent with the scaled solar pure r-process pattern, indicating early r-process enrichment in the Sgr progenitor.

==> author_list.tex <==
%% A significant change from earlier AASTEX versions is in the structure for 
%% calling author and affiliations. The change was necessary to implement 
%% auto-indexing of affiliations which prior was a manual process that could 
%% easily be tedious in large author manuscripts.
%%
%% The \author command is the same as before except it now takes an optional
%% argument which is the 16 digit ORCID. The syntax is:
%% \author[xxxx-xxxx-xxxx-xxxx]{Author Name}
%%
%% This will hyperlink the author name to the author's ORCID page. Note that
%% during compilation, LaTeX will do some limited checking of the format of
%% the ID to make sure it is valid. If the "orcid-ID.png" image file is 
%% present or in the LaTeX pathway, the OrcID icon will appear next to
%% the authors name.
%%
%% Use \affiliation for affiliation information. The old \affil is now aliased
%% to \affiliation. AASTeX v6.31 will automatically index these in the header.
%% When a duplicate is found its index will be the same as its previous entry.
%%
%% Note that \altaffilmark and \altaffiltext have been removed and thus 
%% can not be used to document secondary affiliations. If they are used latex
%% will issue a specific error message and quit. Please use multiple 
%% \affiliation calls for to document more than one affiliation.
%%
%% The new \altaffiliation can be used to indicate some secondary information
%% such as fellowships. This command produces a non-numeric footnote that is
%% set away from the numeric \affiliation footnotes.  NOTE that if an
%% \altaffiliation command is used it must come BEFORE the \affiliation call,
%% right after the \author command, in order to place the footnotes in
%% the proper location.
%%
%% Use \email to set provide email addresses. Each \email will appear on its
%% own line so you can put multiple email address in one \email call. A new
%% \correspondingauthor command is available in V6.31 to identify the
%% corresponding author of the manuscript. It is the author's responsibility
%% to make sure this name is also in the author list.
%%
%% While authors can be grouped inside the same \author and \affiliation
%% commands it is better to have a single author for each. This allows for
%% one to exploit all the new benefits and should make book-keeping easier.
%%
%% If done correctly the peer review system will be able to
%% automatically put the author and affiliation information from the manuscript
%% and save the corresponding author the trouble of entering it by hand.


%% Note that the \and command from previous versions of AASTeX is now
%% depreciated in this version as it is no longer necessary. AASTeX 
%% automatically takes care of all commas and "and"s between authors names.

%% AASTeX 6.31 has the new \collaboration and \nocollaboration commands to
%% provide the collaboration status of a group of authors. These commands 
%% can be used either before or after the list of corresponding authors. The
%% argument for \collaboration is the collaboration identifier. Authors are
%% encouraged to surround collaboration identifiers with ()s. The 
%% \nocollaboration command takes no argument and exists to indicate that
%% the nearby authors are not part of surrounding collaborations.


%\correspondingauthor{August Muench}
%\email{greg.schwarz@aas.org, gus.muench@aas.org}

% \collaboration{20}{(AAS Journals Data Editors)}

%%%%%%%%%%%%%%%%%%%%
% Affiliations

\newcommand{\MITPhysics}{MIT Department of Physics, 
77 Massachusetts Avenue, Cambridge, MA 02139, USA}
\newcommand{\MITKavli}{MIT Kavli Institute for Astrophysics and Space Research, 
77 Massachusetts Avenue, Cambridge, MA 02139, USA}
\newcommand{\UChicagoPhysics}{Department of Astronomy \& Astrophysics, University of Chicago, 5640 S. Ellis Avenue, Chicago, IL 60637, USA}
\newcommand{\UChicagoKavli}{Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}
\newcommand{\USaoPaulo}{Universidade de S\~ao Paulo, Instituto de Astronomia, Geof\'isica e Ci\^encias Atmosf\'ericas, Departamento de Astronomia, SP 05508-090, S\~ao Paulo, Brasil}

%%%%%%%%%%%%%%%%%%%%
% Authors

\author[0000-0002-4669-9967]{Xiaowei Ou}
\affiliation{\MITPhysics}
\affiliation{\MITKavli}

\author[0000-0002-1462-0265]{Alexander Yelland}
\affiliation{\MITPhysics}
\affiliation{\MITKavli}

\author[0000-0002-7155-679X]{Anirudh Chiti}
\affiliation{\UChicagoPhysics}
\affiliation{\UChicagoKavli}

\author[0000-0002-2139-7145]{Anna Frebel}
\affiliation{\MITPhysics}
\affiliation{\MITKavli}

% \author[0000-0002-4863-8842]{Alex Ji}
% \affiliation{\UChicagoPhysics}
% \affiliation{\UChicagoKavli}

\author[0000-0002-9269-8287]{Guilherme Limberg}
\affiliation{\UChicagoPhysics}
\affiliation{\UChicagoKavli}

\author[0000-0001-9178-3992]{Mohammad K.\ Mardini}
\affiliation{\MITKavli}
\affiliation{Department of Physics, Zarqa University, Zarqa 13110, Jordan}
\affiliation{Jordanian Astronomical Virtual Observatory, Zarqa University, Zarqa 13110, Jordan}
\affiliation{Joint Institute for Nuclear Astrophysics -- Center for the Evolution of the Elements (JINA-CEE), USA}


==> tab01.tex <==
% \begin{rotatetable}
\begin{deluxetable*}{lrrrrrlrrrr} 
\tablecaption{Observational Parameters.}
\label{tab:obs_param}
\tabletypesize{\scriptsize}
\tablehead{
    \colhead{Star name} & \colhead{\Gaia\ DR3 Designation} & \colhead{R.A.} & \colhead{Decl.} & \colhead{$\Lambda_{\odot}$} & \colhead{$\rm{B}_{\odot}$} & \colhead{UT Date} & \colhead{$t_{\rm exp}$} & \colhead{$g$} & \colhead{$v_{\rm helio}$} & \colhead{S/N}
    \\
    \colhead{} & \colhead{} & \colhead{(h:m:s)} & \colhead{(d:m:s)} & \colhead{(${\rm deg}$)} & \colhead{(${\rm deg}$)} & \colhead{} & \colhead{(${\rm s}$)} & \colhead{${\rm (mag)}$} & \colhead{(${\rm km \, s^{-1}}$)} & \colhead{}% \hline
}
\startdata
\multicolumn{11}{c}{Stream} \\
\hline
{\large\noFillCircle} Sgr421   & 620763790933951488  & 09:36:00.0 & $+$17:07:21.4 & 216.9 & 11.6   & 2023 May 24 & 1320 & 14.5 & 140.1    & 32, 63 \\
{\large\noFillCircle} Sgr422   & 626434144197068160  & 09:57:30.0 & $+$18:30:17.4 & 221.7 & 9.2    & 2023 May 25 & 4163 & 16.2 & $-$61.8  & 13, 23 \\
{\large\noFillCircle} Sgr423   & 722010223233565952  & 10:21:32.3 & $+$21:46:38.8 & 226.4 & 4.6    & 2023 May 24 & 2100 & 15.0 & $-$42.8  & 32, 62 \\
{\large\noFillCircle} Sgr424   & 720678611573056384  & 10:28:03.8 & $+$20:16:15.9 & 228.3 & 5.7    & 2023 May 25 & 1500 & 15.4 & $-$41.7  & 22, 41 \\
{\large\noFillCircle} Sgr426   & 3987367858589682432 & 10:35:36.8 & $+$20:33:51.4 & 229.9 & 4.9    & 2023 May 25 & 2100 & 15.1 & $-$51.8  & 31, 62 \\
{\large\noFillCircle} Sgr428   & 3897736907644138368 & 11:49:36.0 & $+$06:15:31.9 & 252.0 & 11.8   & 2023 May 25 & 1200 & 15.9 & 193.4    & 19, 35 \\
{\large\noFillCircle} Sgr430   & 3918753557013284608 & 12:05:57.8 & $+$11:26:28.1 & 253.5 & 5.4    & 2023 May 25 & 2106 & 14.7 & $-$18.3  & 35, 82 \\
{\large\noFillCircle} Sgr431   & 3707325064494295552 & 12:36:03.1 & $+$04:22:23.4 & 263.4 & 8.3    & 2023 Jun 25 & 4794 & 16.1 & 9.8      & 18, 40 \\
{\large\noFillCircle} Sgr434   & 3708871630677912320 & 12:48:19.6 & $+$05:44:47.2 & 265.5 & 5.7    & 2023 Jun 25 & 2754 & 15.7 & $-$8.5   & 24, 43 \\
{\large\noFillCircle} Sgr438   & 3742595885684658560 & 13:17:16.3 & $+$12:51:15.1 & 268.3 & $-$4.0 & 2023 May 26 & 3990 & 15.8 & $-$103.0 & 28, 47 \\
{\large\noFillCircle} Sgr441   & 3726554388991980800 & 13:38:16.5 & $+$10:54:19.8 & 273.8 & $-$4.8 & 2023 May 26 & 5999 & 15.4 & $-$22.1  & 20, 51 \\
{\large\noFillCircle} Sgr442   & 3713742742066109568 & 13:39:13.6 & $+$04:20:10.8 & 277.3 & 0.7    & 2023 May 25 & 1800 & 15.2 & 123.2    & 29, 57 \\
{\large\noFillCircle} Sgr449   & 3724011729697503616 & 14:02:29.1 & $+$10:17:36.9 & 279.2 & $-$7.3 & 2023 May 25 & 1537 & 14.7 & $-$140.2 & 36, 66 \\
{\large\noFillCircle} Sgr452   & 3654980335256551808 & 14:34:27.4 & $+$00:57:43.5 & 290.9 & $-$3.3 & 2023 May 25 & 3386 & 16.2 & $-$7.3   & 24, 51 \\
{\large\noFillCircle} Sgr453   & 4415617329687172224 & 15:20:10.2 & $-$00:55:16.2 & 301.8 & $-$7.4 & 2023 Jun 26 & 1500 & 15.1 & $-$216.7 & 17, 41 \\
\hline
\multicolumn{11}{c}{Core} \\
\hline
{\large\fullFillCircle} Sgr459 & 4046752756534194304 & 18:35:35.3 & $-$31:04:52.3 & 356.0 & 2.9    & 2023 Jun 26 & 2400 & 15.1 & 170.3    & 23, 53 \\
{\large\fullFillCircle} Sgr460 & 4046692626988248704 & 18:37:37.0 & $-$31:12:18.7 & 356.5 & 2.9    & 2023 May 25 & 3378 & 15.9 & 154.7    & 26, 54 \\
{\large\fullFillCircle} Sgr462 & 4047106558751402112 & 18:39:44.8 & $-$30:37:02.0 & 356.8 & 2.3    & 2023 May 26 & 3600 & 15.8 & 157.4    & 29, 61 \\
{\large\fullFillCircle} Sgr463 & 4047227809930988288 & 18:43:10.7 & $-$30:13:29.2 & 357.5 & 1.7    & 2023 May 26 & 4435 & 15.0 & 161.7    & 31, 71 \\
{\large\fullFillCircle} Sgr468 & 6732306574448077824 & 18:49:32.1 & $-$34:35:45.8 & 359.6 & 5.8    & 2023 May 26 & 3964 & 15.3 & 135.3    & 30, 68 \\
{\large\fullFillCircle} Sgr2   & 6735720523692986368 & 18:49:59.0 & $-$33:49:51.5 & 359.6 & 5.0    & 2021 Jul 30 & 2673 & 15.3 & 171.9    & 24, 57 \\
{\large\fullFillCircle} Sgr471 & 6736253885603451776 & 18:50:53.7 & $-$31:33:17.7 & 359.3 & 2.7    & 2023 Jun 26 & 3000 & 15.1 & 148.0    & 28, 61 \\
{\large\fullFillCircle} Sgr476 & 6736183692971769472 & 18:52:10.3 & $-$31:54:13.2 & 359.7 & 3.0    & 2023 May 26 & 4307 & 14.9 & 166.1    & 29, 72 \\
{\large\fullFillCircle} Sgr69  & 6761301211485896192 & 18:52:48.5 & $-$29:32:23.4 & 359.4 & 0.7    & 2021 Jul 31 & 600  & 15.1 & 136.8    & 9, 26 \\ 
{\large\fullFillCircle} Sgr482 & 6760843501083241216 & 18:56:40.2 & $-$29:54:02.0 & 0.3   & 0.9    & 2023 May 25 & 2135 & 15.3 & 147.1    & 28, 58 \\
{\large\fullFillCircle} Sgr4   & 6760823641153762816 & 18:57:04.5 & $-$30:10:21.6 & 0.4   & 1.1    & 2021 Jul 30 & 1200 & 14.9 & 140.3    & 17, 47 \\
{\large\fullFillCircle} Sgr38  & 6760148545331944832 & 18:57:27.7 & $-$31:07:39.9 & 0.6   & 2.0    & 2021 Jul 31 & 3225 & 16.0 & 162.2    & 19, 45 \\
{\large\fullFillCircle} Sgr484 & 6756665051965670400 & 19:01:38.9 & $-$32:54:27.2 & 1.8   & 3.7    & 2023 May 25 & 3175 & 15.8 & 159.0    & 27, 55 \\
{\large\fullFillCircle} Sgr488 & 6755741496554745728 & 19:05:13.1 & $-$34:09:16.6 & 2.7   & 4.8    & 2023 May 26 & 2833 & 15.2 & 139.6    & 25, 57 \\
{\large\fullFillCircle} Sgr492 & 6757188660021199360 & 19:06:12.1 & $-$31:55:04.5 & 2.6   & 2.5    & 2023 May 26 & 1200 & 15.2 & 143.7    & 10, 25 \\
{\large\fullFillCircle} Sgr495 & 6757333348879294336 & 19:09:05.2 & $-$31:06:32.8 & 3.1   & 1.6    & 2023 May 25 & 1506 & 14.7 & 157.6    & 29, 67 \\
{\large\fullFillCircle} Sgr496 & 6762312242461355008 & 19:10:57.1 & $-$28:53:15.9 & 3.2   & $-$0.6 & 2023 May 25 & 2602 & 15.7 & 120.6    & 25, 55 \\
{\large\fullFillCircle} Sgr9   & 6756198442417269504 & 19:14:03.2 & $-$32:42:03.5 & 4.4   & 3.1    & 2021 Jul 30 & 2400 & 15.5 & 122.3    & 20, 50 \\
{\large\fullFillCircle} Sgr504 & 6756126841019510784 & 19:14:48.7 & $-$33:07:52.9 & 4.6   & 3.5    & 2023 Jun 26 & 1500 & 15.2 & 148.1    & 24, 47 \\
{\large\fullFillCircle} Sgr505 & 6759005362463205760 & 19:15:12.0 & $-$29:53:26.1 & 4.2   & 0.3    & 2023 Jun 26 & 3000 & 15.3 & 136.0    & 22, 47 \\
{\large\fullFillCircle} Sgr509 & 6744030735644086784 & 19:18:30.2 & $-$33:42:59.7 & 5.4   & 4.0    & 2023 May 25 & 2892 & 15.7 & 169.9    & 30, 59 \\
{\large\fullFillCircle} Sgr512 & 6744069390349796224 & 19:19:57.4 & $-$33:13:50.9 & 5.7   & 3.4    & 2023 May 25 & 2110 & 15.4 & 121.5    & 26, 55   
\enddata
\tablenotetext{}{Stars found in the Sagittarius core are denoted with black-filled circles ({\large\fullFillCircle}), and stars found the Sagittarius streams are denoted with white-filled circles ({\large\noFillCircle}). Signal-to-noise (S/N) per pixel is listed for $4500$ \AA\ and $6500$ \AA.}
% Right ascension (R.A.), declination (Decl.), and $g$ magnitude were measured by \Gaia\ using the J2000 epoch.
\end{deluxetable*}
% \end{rotatetable}

==> tab02.tex <==
\begin{deluxetable*}{lcccccccc}
\tablecaption{Stellar parameters of the 37 Sgr stars in this study.}
\label{tab:ste_par}
\tabletypesize{\scriptsize}
\tablewidth{\linewidth}
\tablehead{
    \colhead{Star Name} & \colhead{$T_{\rm eff}$} & \colhead{$\sigma_{T_{\rm eff}}$} & \colhead{$\log \, g$} & \colhead{$\sigma_{\log \, g}$} & \colhead{$v_{\rm t}$} & \colhead{$\sigma_{v_{\rm t}}$} & \colhead{${\rm [Fe/H]}$} & \colhead{$\sigma_{\rm [Fe/H]}$}
    \\
    \colhead{} & \colhead{(${\rm K}$)} & \colhead{(${\rm K}$)} & \colhead{(${\rm cgs}$)} & \colhead{(${\rm cgs}$)} & \colhead{(${\rm km \, s^{-1}}$)} & \colhead{(${\rm km \, s^{-1}}$)} & \colhead{(${\rm dex}$)} & \colhead{(${\rm dex}$)}}
\startdata
\multicolumn{9}{c}{Stream} \\
\hline
{\large\noFillCircle} Sgr421 & 4655 & 122 & 1.14 & 0.20 & 2.2 & 0.3 & $-$2.81 & 0.16 \\
{\large\noFillCircle} Sgr422 & 5026 & 123 & 2.06 & 0.20 & 1.9 & 0.3 & $-$1.93 & 0.19 \\
{\large\noFillCircle} Sgr423 & 4722 & 122 & 1.29 & 0.20 & 2.1 & 0.3 & $-$2.52 & 0.09 \\
{\large\noFillCircle} Sgr424 & 4814 & 122 & 1.50 & 0.20 & 1.9 & 0.3 & $-$2.43 & 0.17 \\
{\large\noFillCircle} Sgr426 & 4750 & 122 & 1.36 & 0.20 & 2.2 & 0.3 & $-$2.93 & 0.14 \\
{\large\noFillCircle} Sgr428 & 4790 & 123 & 1.48 & 0.20 & 2.2 & 0.3 & $-$2.39 & 0.18 \\
{\large\noFillCircle} Sgr430 & 4280 & 122 & 0.40 & 0.20 & 2.2 & 0.3 & $-$2.42 & 0.21 \\
{\large\noFillCircle} Sgr431 & 4659 & 123 & 1.15 & 0.20 & 2.1 & 0.4 & $-$2.82 & 0.18 \\
{\large\noFillCircle} Sgr434 & 4846 & 123 & 1.57 & 0.20 & 1.9 & 0.3 & $-$2.70 & 0.16 \\
{\large\noFillCircle} Sgr438 & 5274 & 123 & 2.60 & 0.20 & 1.4 & 0.3 & $-$2.53 & 0.16 \\
{\large\noFillCircle} Sgr441 & 4334 & 122 & 0.47 & 0.20 & 2.5 & 0.3 & $-$2.78 & 0.21 \\
{\large\noFillCircle} Sgr442 & 4697 & 122 & 1.24 & 0.20 & 2.0 & 0.3 & $-$3.21 & 0.16 \\
{\large\noFillCircle} Sgr449 & 4759 & 122 & 1.33 & 0.20 & 1.9 & 0.3 & $-$3.29 & 0.15 \\
{\large\noFillCircle} Sgr452 & 4516 & 123 & 0.84 & 0.20 & 2.4 & 0.3 & $-$3.16 & 0.17 \\
{\large\noFillCircle} Sgr453 & 4313 & 122 & 0.59 & 0.21 & 2.1 & 0.3 & $-$2.25 & 0.23 \\
\hline
\multicolumn{9}{c}{Core} \\
\hline
{\large\fullFillCircle} Sgr459 & 4363 & 122 & 0.53 & 0.20 & 2.3 & 0.3 & $-$2.66 & 0.21 \\
{\large\fullFillCircle} Sgr460 & 4717 & 123 & 1.28 & 0.20 & 2.2 & 0.3 & $-$3.00 & 0.16 \\
{\large\fullFillCircle} Sgr462 & 4625 & 122 & 1.07 & 0.20 & 2.2 & 0.3 & $-$2.83 & 0.16 \\
{\large\fullFillCircle} Sgr463 & 4423 & 122 & 0.65 & 0.20 & 2.2 & 0.3 & $-$2.69 & 0.19 \\
{\large\fullFillCircle} Sgr468 & 4491 & 122 & 0.79 & 0.20 & 2.2 & 0.3 & $-$2.57 & 0.20 \\
{\large\fullFillCircle} Sgr2   & 4609 & 122 & 1.04 & 0.20 & 2.2 & 0.3 & $-$2.66 & 0.17 \\
{\large\fullFillCircle} Sgr471 & 4542 & 122 & 0.89 & 0.20 & 2.4 & 0.3 & $-$3.14 & 0.17 \\
{\large\fullFillCircle} Sgr476 & 4371 & 122 & 0.54 & 0.20 & 1.9 & 0.3 & $-$2.88 & 0.22 \\
{\large\fullFillCircle} Sgr69  & 4401 & 122 & 0.60 & 0.20 & 2.5 & 0.3 & $-$2.68 & 0.22 \\
{\large\fullFillCircle} Sgr482 & 4604 & 122 & 1.02 & 0.20 & 2.1 & 0.3 & $-$2.74 & 0.17 \\
{\large\fullFillCircle} Sgr4   & 4379 & 122 & 0.56 & 0.20 & 2.5 & 0.4 & $-$3.10 & 0.19 \\
{\large\fullFillCircle} Sgr38  & 4784 & 123 & 1.43 & 0.20 & 2.0 & 0.3 & $-$2.72 & 0.17 \\
{\large\fullFillCircle} Sgr484 & 4697 & 123 & 1.23 & 0.20 & 2.0 & 0.3 & $-$2.94 & 0.15 \\
{\large\fullFillCircle} Sgr488 & 4492 & 122 & 0.79 & 0.20 & 2.3 & 0.3 & $-$3.02 & 0.20 \\
{\large\fullFillCircle} Sgr492 & 4466 & 122 & 0.73 & 0.20 & 2.5 & 0.6 & $-$2.81 & 0.25 \\
{\large\fullFillCircle} Sgr495 & 4412 & 122 & 0.63 & 0.20 & 2.3 & 0.3 & $-$2.96 & 0.17 \\
{\large\fullFillCircle} Sgr496 & 4613 & 122 & 1.04 & 0.20 & 1.9 & 0.3 & $-$2.95 & 0.18 \\
{\large\fullFillCircle} Sgr9   & 4589 & 122 & 1.30 & 0.20 & 2.1 & 0.3 & $-$1.85 & 0.20 \\
{\large\fullFillCircle} Sgr504 & 4517 & 122 & 0.84 & 0.20 & 2.2 & 0.3 & $-$2.67 & 0.19 \\
{\large\fullFillCircle} Sgr505 & 4524 & 122 & 0.85 & 0.20 & 2.2 & 0.3 & $-$3.06 & 0.17 \\
{\large\fullFillCircle} Sgr509 & 4699 & 122 & 1.24 & 0.20 & 2.0 & 0.3 & $-$3.18 & 0.16 \\
{\large\fullFillCircle} Sgr512 & 4614 & 122 & 1.05 & 0.20 & 2.0 & 0.3 & $-$3.03 & 0.16   
\enddata
% \tablenotetext{}{}
\end{deluxetable*}


==> tab03.tex <==
\begin{deluxetable*}{lrrrrrrr} 
\tablecaption{Chemical Abundances.}
\label{tab:abundances}
\tabletypesize{\scriptsize}
\tablehead{\colhead{El.} & \colhead{N} & \colhead{$\log \epsilon (\rm{X})_{\*}$} & \colhead{$\sigma$} & \colhead{${\rm [X/H]}$} & \colhead{$\sigma_{\rm [X/H]}$} & \colhead{${\rm [X/Fe]}$} & \colhead{$\sigma_{\rm [X/Fe]}$}}
\startdata
\multicolumn{8}{c}{Sgr2} \\ \hline
Na I  & 2   & 3.96    & 0.07      & $-$2.28 & 0.25      & 0.38    & 0.12 \\     
Mg I  & 4   & 5.25    & 0.13      & $-$2.35 & 0.16      & 0.31    & 0.08 \\     
Al I  & 2   & 3.37    & 0.22      & $-$3.09 & 0.42      & $-$0.43 & 0.29 \\     
Si I  & 2   & 5.34    & 0.21      & $-$2.17 & 0.26      & 0.49    & 0.16 \\     
Ca I  & 15  & 3.97    & 0.16      & $-$2.37 & 0.13      & 0.29    & 0.06 \\     
Sc II & 7   & 0.52    & 0.12      & $-$2.63 & 0.10      & $-$0.08 & 0.06 \\     
Ti I  & 14  & 2.30    & 0.17      & $-$2.65 & 0.20      & 0.01    & 0.07 \\     
Ti II & 29  & 2.57    & 0.15      & $-$2.38 & 0.12      & 0.17    & 0.07 \\     
V I   & 2   & 0.95    & 0.01      & $-$2.99 & 0.12      & $-$0.33 & 0.10 \\     
V II  & 2   & 1.16    & 0.10      & $-$2.77 & 0.10      & $-$0.22 & 0.11 \\     
Cr I  & 9   & 2.80    & 0.12      & $-$2.84 & 0.19      & $-$0.19 & 0.05 \\     
Cr II & 3   & 3.07    & 0.14      & $-$2.57 & 0.11      & $-$0.02 & 0.10 \\     
Mn I  & 6   & 2.27    & 0.08      & $-$3.16 & 0.11      & $-$0.51 & 0.09 \\     
Fe I  & 154 & 4.84    & 0.20      & $-$2.66 & 0.17      & 0.00    & 0.00 \\     
Fe II & 15  & 4.95    & 0.12      & $-$2.55 & 0.10      & 0.00    & 0.00 \\     
Co I  & 4   & 2.29    & 0.21      & $-$2.70 & 0.17      & $-$0.04 & 0.12 \\     
Ni I  & 4   & 3.59    & 0.21      & $-$2.63 & 0.24      & 0.03    & 0.12 \\     
Zn I  & 1   & 2.06    & 0.00      & $-$2.50 & 0.06      & 0.16    & 0.13 \\     
Sr II & 2   & 0.61    & 0.11      & $-$2.26 & 0.18      & 0.29    & 0.15 \\     
Y II  & 3   & $-$0.59 & 0.07      & $-$2.80 & 0.10      & $-$0.25 & 0.09 \\     
Zr II & 1   & 0.14    & 0.00      & $-$2.44 & 0.10      & 0.11    & 0.06 \\     
Ba II & 5   & $-$0.94 & 0.17      & $-$3.12 & 0.13      & $-$0.57 & 0.10 \\     
La II & 3   & $-$1.94 & 0.10      & $-$3.04 & 0.10      & $-$0.49 & 0.13 \\     
C$-$H & 2   & 5.44    & 0.01      & $-$2.99 & 0.29      & $-$0.34 & 0.19 \\     
C$-$N & 1   & 6.22    & 0.00      & $-$1.61 & 0.40      & 1.05    & 0.27 \\     
Eu II & 3   & $-$2.27 & $\nodata$ & $-$2.79 & $\nodata$ & $-$0.23 & $\nodata$ \\
Dy II & 1   & $-$0.60 & $\nodata$ & $-$1.70 & $\nodata$ & 0.86    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr4} \\ \hline
Na I  & 2   & 3.48    & 0.03      & $-$2.76 & 0.31      & 0.34    & 0.16 \\     
Mg I  & 4   & 4.90    & 0.13      & $-$2.70 & 0.19      & 0.40    & 0.07 \\     
Al I  & 1   & 2.44    & 0.00      & $-$4.01 & 0.24      & $-$0.91 & 0.08 \\     
Si I  & 1   & 4.93    & 0.00      & $-$2.58 & 0.25      & 0.52    & 0.10 \\     
Ca I  & 14  & 3.63    & 0.19      & $-$2.71 & 0.14      & 0.39    & 0.08 \\     
Sc II & 7   & 0.09    & 0.16      & $-$3.06 & 0.12      & 0.04    & 0.07 \\     
Ti I  & 13  & 1.97    & 0.22      & $-$2.98 & 0.22      & 0.12    & 0.08 \\     
Ti II & 24  & 2.16    & 0.15      & $-$2.79 & 0.16      & 0.31    & 0.09 \\     
V I   & 2   & 0.55    & 0.19      & $-$3.38 & 0.19      & $-$0.28 & 0.18 \\     
V II  & 2   & 0.96    & 0.09      & $-$2.97 & 0.16      & 0.12    & 0.10 \\     
Cr I  & 6   & 2.10    & 0.29      & $-$3.54 & 0.25      & $-$0.44 & 0.13 \\     
Mn I  & 4   & 1.93    & 0.06      & $-$3.50 & 0.12      & $-$0.40 & 0.09 \\     
Fe I  & 128 & 4.40    & 0.23      & $-$3.10 & 0.19      & 0.00    & 0.00 \\     
Fe II & 15  & 4.40    & 0.10      & $-$3.10 & 0.12      & 0.00    & 0.00 \\     
Co I  & 4   & 1.89    & 0.26      & $-$3.10 & 0.21      & 0.00    & 0.14 \\     
Ni I  & 3   & 3.24    & 0.07      & $-$2.98 & 0.20      & 0.12    & 0.06 \\     
Zn I  & 1   & 1.84    & 0.00      & $-$2.73 & 0.07      & 0.38    & 0.17 \\     
Sr II & 2   & $-$0.34 & 0.04      & $-$3.21 & 0.34      & $-$0.12 & 0.28 \\     
Y II  & 3   & $-$1.18 & 0.06      & $-$3.39 & 0.15      & $-$0.29 & 0.09 \\     
Zr II & 1   & $-$0.37 & 0.00      & $-$2.95 & 0.14      & 0.15    & 0.07 \\     
Ba II & 5   & $-$2.08 & 0.16      & $-$4.26 & 0.16      & $-$1.16 & 0.11 \\     
C$-$H & 2   & 4.48    & 0.00      & $-$3.95 & 0.33      & $-$0.85 & 0.28 \\     
C$-$N & 1   & 5.51    & 0.00      & $-$2.32 & 0.34      & 0.78    & 0.32 \\     
La II & 3   & $-$1.94 & $\nodata$ & $-$3.04 & $\nodata$ & 0.06    & $\nodata$ \\
Eu II & 2   & $-$2.34 & $\nodata$ & $-$2.86 & $\nodata$ & 0.24    & $\nodata$ \\
Dy II & 2   & $-$1.58 & $\nodata$ & $-$2.68 & $\nodata$ & 0.41    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr9} \\ \hline
Na I  & 2   & 4.42    & 0.10 & $-$1.82 & 0.27 & 0.02    & 0.10 \\
Mg I  & 3   & 5.85    & 0.04 & $-$1.75 & 0.18 & 0.10    & 0.09 \\
Al I  & 2   & 3.93    & 0.17 & $-$2.52 & 0.50 & $-$0.67 & 0.39 \\
Si I  & 2   & 6.00    & 0.15 & $-$1.51 & 0.19 & 0.34    & 0.12 \\
Ca I  & 25  & 4.86    & 0.13 & $-$1.48 & 0.15 & 0.37    & 0.07 \\
Sc II & 6   & 1.44    & 0.29 & $-$1.71 & 0.18 & $-$0.03 & 0.13 \\
Ti I  & 14  & 3.20    & 0.20 & $-$1.75 & 0.26 & 0.10    & 0.09 \\
Ti II & 26  & 3.68    & 0.31 & $-$1.28 & 0.19 & 0.41    & 0.11 \\
V I   & 1   & 1.91    & 0.00 & $-$2.02 & 0.15 & $-$0.18 & 0.12 \\
V II  & 2   & 2.43    & 0.15 & $-$1.50 & 0.15 & 0.19    & 0.15 \\
Cr I  & 9   & 3.63    & 0.18 & $-$2.01 & 0.25 & $-$0.17 & 0.08 \\
Cr II & 3   & 4.01    & 0.17 & $-$1.64 & 0.15 & 0.05    & 0.12 \\
Mn I  & 6   & 3.11    & 0.14 & $-$2.32 & 0.14 & $-$0.48 & 0.12 \\
Fe I  & 164 & 5.65    & 0.20 & $-$1.85 & 0.20 & 0.00    & 0.00 \\
Fe II & 14  & 5.81    & 0.21 & $-$1.69 & 0.15 & 0.00    & 0.00 \\
Co I  & 4   & 3.20    & 0.50 & $-$1.79 & 0.30 & 0.06    & 0.25 \\
Ni I  & 9   & 4.17    & 0.17 & $-$2.05 & 0.14 & $-$0.20 & 0.11 \\
Cu I  & 1   & 1.58    & 0.00 & $-$2.62 & 0.18 & $-$0.77 & 0.10 \\
Zn I  & 1   & 2.77    & 0.00 & $-$1.79 & 0.08 & 0.06    & 0.23 \\
Sr II & 2   & 1.21    & 0.12 & $-$1.66 & 0.13 & 0.03    & 0.15 \\
Y II  & 1   & 0.20    & 0.00 & $-$2.01 & 0.07 & $-$0.33 & 0.11 \\
Zr II & 1   & 1.12    & 0.00 & $-$1.46 & 0.19 & 0.22    & 0.11 \\
Ba II & 5   & 0.68    & 0.11 & $-$1.50 & 0.18 & 0.18    & 0.12 \\
La II & 3   & $-$0.37 & 0.11 & $-$1.47 & 0.12 & 0.22    & 0.12 \\
Eu II & 3   & $-$0.59 & 0.02 & $-$1.11 & 0.10 & 0.58    & 0.16 \\
Dy II & 2   & 0.03    & 0.12 & $-$1.07 & 0.10 & 0.62    & 0.14 \\
C$-$H & 2   & 5.94    & 0.01 & $-$2.49 & 0.19 & $-$0.64 & 0.21 \\
C$-$N & 1   & 6.49    & 0.00 & $-$1.34 & 0.27 & 0.51    & 0.22 \\
\hline \multicolumn{8}{c}{Sgr38} \\ \hline
Na I  & 2   & 3.69    & 0.10      & $-$2.55 & 0.26      & 0.17    & 0.12 \\     
Mg I  & 5   & 5.32    & 0.26      & $-$2.28 & 0.19      & 0.44    & 0.12 \\     
Al I  & 1   & 3.14    & 0.00      & $-$3.32 & 0.10      & $-$0.59 & 0.15 \\     
Si I  & 2   & 5.25    & 0.17      & $-$2.27 & 0.26      & 0.46    & 0.14 \\     
Ca I  & 15  & 3.82    & 0.21      & $-$2.52 & 0.13      & 0.20    & 0.08 \\     
Sc II & 7   & 0.16    & 0.12      & $-$2.99 & 0.11      & $-$0.43 & 0.08 \\     
Ti I  & 7   & 2.39    & 0.24      & $-$2.56 & 0.20      & 0.16    & 0.10 \\     
Ti II & 19  & 2.42    & 0.12      & $-$2.53 & 0.13      & 0.03    & 0.09 \\     
V I   & 3   & 0.84    & 0.21      & $-$3.09 & 0.44      & $-$0.37 & 0.35 \\     
Cr I  & 7   & 2.66    & 0.25      & $-$2.98 & 0.21      & $-$0.26 & 0.10 \\     
Cr II & 1   & 2.91    & 0.00      & $-$2.73 & 0.08      & $-$0.18 & 0.08 \\     
Mn I  & 5   & 2.29    & 0.05      & $-$3.14 & 0.10      & $-$0.42 & 0.10 \\     
Fe I  & 143 & 4.78    & 0.21      & $-$2.72 & 0.17      & 0.00    & 0.00 \\     
Fe II & 16  & 4.94    & 0.23      & $-$2.56 & 0.11      & 0.00    & 0.00 \\     
Co I  & 4   & 2.19    & 0.16      & $-$2.80 & 0.16      & $-$0.07 & 0.10 \\     
Ni I  & 3   & 3.73    & 0.16      & $-$2.49 & 0.25      & 0.24    & 0.12 \\     
Zn I  & 1   & 2.28    & 0.00      & $-$2.28 & 0.06      & 0.44    & 0.14 \\     
Sr II & 2   & 0.93    & 0.16      & $-$1.94 & 0.18      & 0.62    & 0.17 \\     
Y II  & 3   & $-$0.37 & 0.01      & $-$2.58 & 0.08      & $-$0.02 & 0.08 \\     
Zr II & 1   & 0.10    & 0.00      & $-$2.48 & 0.11      & 0.08    & 0.09 \\     
Ba II & 5   & $-$1.34 & 0.16      & $-$3.52 & 0.12      & $-$0.96 & 0.11 \\     
C$-$H & 2   & 5.59    & 0.02      & $-$2.84 & 0.27      & $-$0.12 & 0.15 \\     
C$-$N & 1   & 5.68    & 0.00      & $-$2.15 & 0.35      & 0.58    & 0.28 \\     
La II & 1   & $-$1.51 & $\nodata$ & $-$2.61 & $\nodata$ & $-$0.05 & $\nodata$ \\
Eu II & 3   & $-$2.08 & $\nodata$ & $-$2.60 & $\nodata$ & $-$0.05 & $\nodata$ \\
Dy II & 1   & $-$0.62 & $\nodata$ & $-$1.72 & $\nodata$ & 0.84    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr69} \\ \hline
Na I  & 2   & 3.45    & 0.08      & $-$2.79 & 0.33      & $-$0.11 & 0.14 \\     
Mg I  & 3   & 5.26    & 0.19      & $-$2.34 & 0.25      & 0.34    & 0.12 \\     
Al I  & 1   & 2.69    & 0.00      & $-$3.77 & 0.17      & $-$1.09 & 0.14 \\     
Si I  & 1   & 5.21    & 0.00      & $-$2.30 & 0.18      & 0.37    & 0.07 \\     
Ca I  & 9   & 3.99    & 0.16      & $-$2.36 & 0.17      & 0.32    & 0.09 \\     
Sc II & 8   & 0.63    & 0.22      & $-$2.52 & 0.15      & 0.11    & 0.11 \\     
Ti I  & 5   & 2.43    & 0.21      & $-$2.52 & 0.27      & 0.16    & 0.11 \\     
Ti II & 23  & 2.58    & 0.31      & $-$2.38 & 0.16      & 0.26    & 0.13 \\     
V I   & 2   & 1.24    & 0.20      & $-$2.69 & 0.23      & $-$0.01 & 0.17 \\     
V II  & 3   & 1.49    & 0.06      & $-$2.44 & 0.09      & 0.20    & 0.09 \\     
Cr I  & 6   & 2.75    & 0.24      & $-$2.89 & 0.32      & $-$0.21 & 0.14 \\     
Mn I  & 5   & 2.27    & 0.24      & $-$3.16 & 0.15      & $-$0.49 & 0.17 \\     
Fe I  & 115 & 4.82    & 0.27      & $-$2.68 & 0.22      & 0.00    & 0.00 \\     
Fe II & 11  & 4.86    & 0.24      & $-$2.64 & 0.13      & 0.00    & 0.00 \\     
Co I  & 2   & 2.89    & 0.27      & $-$2.10 & 0.35      & 0.58    & 0.42 \\     
Ni I  & 2   & 3.57    & 0.06      & $-$2.65 & 0.24      & 0.02    & 0.06 \\     
Zn I  & 1   & 2.35    & 0.00      & $-$2.21 & 0.05      & 0.47    & 0.21 \\     
Sr II & 2   & 0.21    & 0.15      & $-$2.66 & 0.20      & $-$0.03 & 0.16 \\     
Y II  & 3   & $-$0.80 & 0.30      & $-$3.01 & 0.19      & $-$0.38 & 0.20 \\     
Ba II & 5   & $-$0.93 & 0.21      & $-$3.11 & 0.15      & $-$0.47 & 0.14 \\     
Eu II & 1   & $-$2.25 & 0.00      & $-$2.77 & 0.10      & $-$0.13 & 0.14 \\     
C$-$H & 2   & 5.06    & 0.04      & $-$3.37 & 0.23      & $-$0.69 & 0.17 \\     
Zr II & 1   & 0.09    & $\nodata$ & $-$2.49 & $\nodata$ & 0.15    & $\nodata$ \\
La II & 3   & $-$1.27 & $\nodata$ & $-$2.37 & $\nodata$ & 0.27    & $\nodata$ \\
Dy II & 1   & $-$0.35 & $\nodata$ & $-$1.45 & $\nodata$ & 1.19    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr421} \\ \hline
Na I  & 2   & 3.77    & 0.02 & $-$2.47 & 0.22 & 0.34    & 0.11 \\
Mg I  & 5   & 5.29    & 0.12 & $-$2.31 & 0.14 & 0.50    & 0.07 \\
Al I  & 2   & 3.09    & 0.17 & $-$3.36 & 0.28 & $-$0.55 & 0.16 \\
Si I  & 2   & 5.25    & 0.05 & $-$2.26 & 0.19 & 0.55    & 0.06 \\
Ca I  & 11  & 3.83    & 0.12 & $-$2.51 & 0.11 & 0.30    & 0.06 \\
Sc II & 8   & 0.38    & 0.07 & $-$2.77 & 0.11 & 0.11    & 0.04 \\
Ti I  & 14  & 2.29    & 0.14 & $-$2.66 & 0.19 & 0.14    & 0.06 \\
Ti II & 27  & 2.46    & 0.14 & $-$2.49 & 0.13 & 0.40    & 0.07 \\
V I   & 3   & 0.97    & 0.05 & $-$2.96 & 0.22 & $-$0.16 & 0.12 \\
V II  & 2   & 1.25    & 0.05 & $-$2.68 & 0.09 & 0.21    & 0.07 \\
Cr I  & 6   & 2.60    & 0.12 & $-$3.04 & 0.17 & $-$0.23 & 0.06 \\
Cr II & 1   & 2.88    & 0.00 & $-$2.76 & 0.08 & 0.12    & 0.05 \\
Mn I  & 6   & 2.05    & 0.08 & $-$3.38 & 0.11 & $-$0.57 & 0.08 \\
Fe I  & 161 & 4.69    & 0.19 & $-$2.81 & 0.16 & 0.00    & 0.00 \\
Fe II & 15  & 4.62    & 0.10 & $-$2.88 & 0.09 & 0.00    & 0.00 \\
Co I  & 4   & 2.43    & 0.23 & $-$2.56 & 0.18 & 0.24    & 0.12 \\
Ni I  & 3   & 3.65    & 0.12 & $-$2.57 & 0.16 & 0.24    & 0.08 \\
Zn I  & 1   & 1.86    & 0.00 & $-$2.70 & 0.06 & 0.11    & 0.13 \\
Sr II & 2   & 0.24    & 0.01 & $-$2.63 & 0.24 & 0.25    & 0.21 \\
Y II  & 3   & $-$0.51 & 0.08 & $-$2.72 & 0.12 & 0.17    & 0.08 \\
Zr II & 1   & 0.02    & 0.00 & $-$2.56 & 0.09 & 0.32    & 0.05 \\
Ba II & 5   & $-$0.23 & 0.04 & $-$2.41 & 0.17 & 0.47    & 0.13 \\
La II & 4   & $-$1.09 & 0.11 & $-$2.19 & 0.12 & 0.69    & 0.08 \\
Eu II & 2   & $-$1.23 & 0.01 & $-$1.75 & 0.09 & 1.14    & 0.06 \\
Dy II & 2   & $-$0.52 & 0.17 & $-$1.62 & 0.14 & 1.27    & 0.14 \\
C$-$H & 2   & 5.30    & 0.04 & $-$3.14 & 0.29 & $-$0.33 & 0.18 \\
C$-$N & 1   & 5.68    & 0.00 & $-$2.15 & 0.34 & 0.65    & 0.23 \\
\hline \multicolumn{8}{c}{Sgr423} \\ \hline
Na I  & 2   & 4.00    & 0.00 & $-$2.25 & 0.16 & 0.27    & 0.09 \\
Mg I  & 5   & 5.40    & 0.14 & $-$2.20 & 0.09 & 0.31    & 0.09 \\
Al I  & 2   & 3.30    & 0.05 & $-$3.15 & 0.13 & $-$0.64 & 0.11 \\
Si I  & 2   & 5.45    & 0.20 & $-$2.07 & 0.16 & 0.45    & 0.15 \\
Ca I  & 16  & 4.14    & 0.11 & $-$2.20 & 0.06 & 0.32    & 0.04 \\
Sc II & 8   & 0.77    & 0.11 & $-$2.39 & 0.11 & 0.11    & 0.06 \\
Ti I  & 16  & 2.56    & 0.14 & $-$2.39 & 0.08 & 0.12    & 0.05 \\
Ti II & 29  & 2.76    & 0.12 & $-$2.19 & 0.11 & 0.30    & 0.06 \\
V I   & 3   & 1.39    & 0.12 & $-$2.54 & 0.10 & $-$0.02 & 0.11 \\
V II  & 2   & 1.56    & 0.05 & $-$2.37 & 0.06 & 0.13    & 0.07 \\
Cr I  & 10  & 2.90    & 0.17 & $-$2.74 & 0.11 & $-$0.22 & 0.06 \\
Cr II & 3   & 3.10    & 0.12 & $-$2.54 & 0.09 & $-$0.04 & 0.09 \\
Mn I  & 6   & 2.43    & 0.10 & $-$3.00 & 0.05 & $-$0.49 & 0.09 \\
Fe I  & 182 & 4.98    & 0.22 & $-$2.52 & 0.09 & 0.00    & 0.00 \\
Fe II & 15  & 5.01    & 0.13 & $-$2.50 & 0.08 & 0.00    & 0.00 \\
Co I  & 4   & 2.67    & 0.13 & $-$2.33 & 0.10 & 0.19    & 0.07 \\
Ni I  & 7   & 3.72    & 0.17 & $-$2.51 & 0.09 & 0.01    & 0.08 \\
Zn I  & 1   & 2.16    & 0.00 & $-$2.40 & 0.04 & 0.11    & 0.06 \\
Sr II & 2   & 0.28    & 0.06 & $-$2.59 & 0.22 & $-$0.09 & 0.16 \\
Y II  & 3   & $-$0.69 & 0.06 & $-$2.90 & 0.08 & $-$0.40 & 0.07 \\
Zr II & 1   & 0.01    & 0.00 & $-$2.57 & 0.07 & $-$0.07 & 0.07 \\
Ba II & 5   & $-$0.75 & 0.07 & $-$2.93 & 0.08 & $-$0.44 & 0.05 \\
La II & 2   & $-$1.29 & 0.02 & $-$2.39 & 0.07 & 0.10    & 0.09 \\
Eu II & 2   & $-$1.74 & 0.05 & $-$2.26 & 0.08 & 0.24    & 0.08 \\
Dy II & 2   & $-$1.16 & 0.10 & $-$2.26 & 0.10 & 0.24    & 0.08 \\
C$-$H & 2   & 5.62    & 0.03 & $-$2.81 & 0.10 & $-$0.29 & 0.15 \\
C$-$N & 1   & 6.05    & 0.00 & $-$1.78 & 0.08 & 0.73    & 0.13 \\
\hline \multicolumn{8}{c}{Sgr426} \\ \hline
Na I  & 2   & 3.42    & 0.17      & $-$2.82 & 0.23      & 0.11    & 0.15 \\     
Mg I  & 5   & 4.99    & 0.10      & $-$2.61 & 0.13      & 0.32    & 0.06 \\     
Al I  & 2   & 2.80    & 0.01      & $-$3.66 & 0.27      & $-$0.72 & 0.15 \\     
Si I  & 2   & 4.98    & 0.01      & $-$2.53 & 0.22      & 0.41    & 0.08 \\     
Ca I  & 14  & 3.60    & 0.17      & $-$2.75 & 0.11      & 0.19    & 0.06 \\     
Sc II & 8   & 0.16    & 0.10      & $-$3.00 & 0.09      & $-$0.14 & 0.06 \\     
Ti I  & 9   & 2.07    & 0.12      & $-$2.88 & 0.16      & 0.05    & 0.06 \\     
Ti II & 25  & 2.18    & 0.16      & $-$2.77 & 0.11      & 0.08    & 0.07 \\     
V I   & 2   & 0.05    & 0.57      & $-$3.88 & 0.41      & $-$0.95 & 0.42 \\     
V II  & 2   & 0.96    & 0.03      & $-$2.97 & 0.10      & $-$0.12 & 0.10 \\     
Cr I  & 5   & 2.43    & 0.21      & $-$3.21 & 0.18      & $-$0.28 & 0.10 \\     
Cr II & 2   & 2.75    & 0.10      & $-$2.89 & 0.10      & $-$0.04 & 0.09 \\     
Mn I  & 6   & 1.93    & 0.20      & $-$3.50 & 0.12      & $-$0.57 & 0.11 \\     
Fe I  & 151 & 4.57    & 0.20      & $-$2.93 & 0.14      & 0.00    & 0.00 \\     
Fe II & 15  & 4.65    & 0.16      & $-$2.85 & 0.08      & 0.00    & 0.00 \\     
Co I  & 4   & 2.14    & 0.16      & $-$2.85 & 0.15      & 0.08    & 0.09 \\     
Ni I  & 3   & 3.26    & 0.07      & $-$2.96 & 0.17      & $-$0.03 & 0.07 \\     
Zn I  & 1   & 1.69    & 0.00      & $-$2.87 & 0.05      & 0.06    & 0.10 \\     
Sr II & 2   & $-$0.49 & 0.01      & $-$3.36 & 0.27      & $-$0.51 & 0.24 \\     
Y II  & 3   & $-$1.07 & 0.16      & $-$3.28 & 0.11      & $-$0.43 & 0.11 \\     
Ba II & 5   & $-$1.36 & 0.08      & $-$3.54 & 0.10      & $-$0.69 & 0.08 \\     
Eu II & 1   & $-$2.25 & 0.00      & $-$2.77 & 0.08      & 0.08    & 0.06 \\     
C$-$H & 2   & 5.52    & 0.00      & $-$2.91 & 0.30      & 0.02    & 0.19 \\     
C$-$N & 1   & 5.87    & 0.00      & $-$1.96 & 0.38      & 0.97    & 0.27 \\     
Zr II & 1   & $-$0.14 & $\nodata$ & $-$2.72 & $\nodata$ & 0.13    & $\nodata$ \\
La II & 1   & $-$1.24 & $\nodata$ & $-$2.34 & $\nodata$ & 0.51    & $\nodata$ \\
Dy II & 2   & $-$1.16 & $\nodata$ & $-$2.26 & $\nodata$ & 0.60    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr428} \\ \hline
Na I  & 2   & 4.08    & 0.01 & $-$2.16 & 0.25 & 0.23    & 0.09 \\
Mg I  & 4   & 5.47    & 0.09 & $-$2.13 & 0.16 & 0.26    & 0.07 \\
Al I  & 2   & 3.14    & 0.36 & $-$3.31 & 0.37 & $-$0.92 & 0.28 \\
Si I  & 1   & 5.47    & 0.00 & $-$2.04 & 0.20 & 0.35    & 0.07 \\
Ca I  & 17  & 4.21    & 0.17 & $-$2.13 & 0.13 & 0.26    & 0.07 \\
Sc II & 8   & 1.04    & 0.19 & $-$2.11 & 0.15 & 0.23    & 0.09 \\
Ti I  & 16  & 2.60    & 0.18 & $-$2.35 & 0.18 & 0.04    & 0.07 \\
Ti II & 21  & 2.90    & 0.18 & $-$2.05 & 0.15 & 0.29    & 0.09 \\
V I   & 3   & 1.42    & 0.06 & $-$2.51 & 0.20 & $-$0.12 & 0.12 \\
V II  & 2   & 1.74    & 0.10 & $-$2.19 & 0.11 & 0.15    & 0.11 \\
Cr I  & 7   & 2.96    & 0.12 & $-$2.68 & 0.20 & $-$0.29 & 0.05 \\
Cr II & 3   & 3.30    & 0.06 & $-$2.34 & 0.09 & 0.00    & 0.07 \\
Mn I  & 6   & 2.61    & 0.06 & $-$2.82 & 0.10 & $-$0.43 & 0.11 \\
Fe I  & 175 & 5.11    & 0.24 & $-$2.39 & 0.18 & 0.00    & 0.00 \\
Fe II & 15  & 5.16    & 0.13 & $-$2.34 & 0.11 & 0.00    & 0.00 \\
Co I  & 4   & 2.72    & 0.25 & $-$2.27 & 0.18 & 0.12    & 0.14 \\
Ni I  & 6   & 3.87    & 0.16 & $-$2.35 & 0.15 & 0.04    & 0.09 \\
Zn I  & 1   & 2.18    & 0.00 & $-$2.38 & 0.06 & 0.01    & 0.15 \\
Sr II & 2   & 0.31    & 0.05 & $-$2.56 & 0.30 & $-$0.22 & 0.23 \\
Y II  & 3   & $-$0.38 & 0.06 & $-$2.59 & 0.11 & $-$0.25 & 0.09 \\
Zr II & 1   & 0.28    & 0.00 & $-$2.30 & 0.08 & 0.04    & 0.08 \\
Ba II & 5   & $-$0.10 & 0.14 & $-$2.28 & 0.18 & 0.06    & 0.12 \\
La II & 3   & $-$1.02 & 0.08 & $-$2.12 & 0.10 & 0.21    & 0.09 \\
Eu II & 2   & $-$1.18 & 0.04 & $-$1.70 & 0.12 & 0.64    & 0.11 \\
Dy II & 2   & $-$0.28 & 0.02 & $-$1.38 & 0.07 & 0.96    & 0.07 \\
C$-$H & 2   & 5.37    & 0.10 & $-$3.06 & 0.26 & $-$0.67 & 0.20 \\
C$-$N & 1   & 5.66    & 0.00 & $-$2.17 & 0.22 & 0.22    & 0.39 \\
\hline \multicolumn{8}{c}{Sgr430} \\ \hline
Na I  & 2   & 4.26    & 0.09 & $-$1.99 & 0.32 & 0.44    & 0.13 \\
Mg I  & 4   & 5.55    & 0.04 & $-$2.05 & 0.18 & 0.37    & 0.07 \\
Al I  & 2   & 3.38    & 0.14 & $-$3.07 & 0.42 & $-$0.65 & 0.26 \\
Si I  & 2   & 5.25    & 0.21 & $-$2.26 & 0.22 & 0.16    & 0.16 \\
Ca I  & 26  & 4.23    & 0.15 & $-$2.11 & 0.16 & 0.31    & 0.06 \\
Sc II & 7   & 0.88    & 0.17 & $-$2.27 & 0.14 & 0.01    & 0.08 \\
Ti I  & 18  & 2.58    & 0.09 & $-$2.37 & 0.35 & 0.05    & 0.15 \\
Ti II & 27  & 2.98    & 0.26 & $-$1.97 & 0.15 & 0.31    & 0.11 \\
V I   & 1   & 1.34    & 0.00 & $-$2.59 & 0.24 & $-$0.17 & 0.08 \\
V II  & 2   & 1.78    & 0.13 & $-$2.16 & 0.16 & 0.12    & 0.14 \\
Cr I  & 9   & 3.12    & 0.12 & $-$2.52 & 0.30 & $-$0.10 & 0.09 \\
Cr II & 3   & 3.26    & 0.15 & $-$2.38 & 0.13 & $-$0.10 & 0.12 \\
Mn I  & 6   & 2.76    & 0.08 & $-$2.67 & 0.15 & $-$0.25 & 0.09 \\
Fe I  & 177 & 5.08    & 0.14 & $-$2.42 & 0.21 & 0.00    & 0.00 \\
Fe II & 16  & 5.22    & 0.20 & $-$2.28 & 0.13 & 0.00    & 0.00 \\
Co I  & 4   & 2.68    & 0.20 & $-$2.31 & 0.21 & 0.11    & 0.11 \\
Ni I  & 11  & 3.72    & 0.11 & $-$2.50 & 0.17 & $-$0.08 & 0.06 \\
Cu I  & 1   & 0.67    & 0.00 & $-$3.53 & 0.14 & $-$1.10 & 0.12 \\
Zn I  & 1   & 2.06    & 0.00 & $-$2.51 & 0.05 & $-$0.08 & 0.24 \\
Sr II & 2   & 0.50    & 0.05 & $-$2.37 & 0.12 & $-$0.09 & 0.11 \\
Y II  & 3   & $-$0.72 & 0.07 & $-$2.93 & 0.10 & $-$0.65 & 0.11 \\
Zr II & 1   & $-$0.01 & 0.00 & $-$2.59 & 0.11 & $-$0.31 & 0.10 \\
Ba II & 5   & $-$0.66 & 0.08 & $-$2.84 & 0.13 & $-$0.56 & 0.10 \\
La II & 4   & $-$1.56 & 0.10 & $-$2.66 & 0.11 & $-$0.38 & 0.13 \\
Eu II & 2   & $-$1.83 & 0.00 & $-$2.35 & 0.09 & $-$0.07 & 0.13 \\
Dy II & 2   & $-$1.08 & 0.03 & $-$2.18 & 0.07 & 0.10    & 0.10 \\
C$-$H & 2   & 5.15    & 0.04 & $-$3.28 & 0.24 & $-$0.86 & 0.22 \\
C$-$N & 1   & 5.62    & 0.00 & $-$2.21 & 0.24 & 0.21    & 0.23 \\
\hline \multicolumn{8}{c}{Sgr449} \\ \hline
Na I  & 2   & 3.86    & 0.16      & $-$2.38 & 0.28      & 0.91    & 0.18 \\     
Mg I  & 3   & 4.33    & 0.10      & $-$3.27 & 0.18      & 0.02    & 0.09 \\     
Al I  & 2   & 3.32    & 0.07      & $-$3.14 & 0.26      & 0.15    & 0.15 \\     
Si I  & 2   & 5.15    & 0.04      & $-$2.36 & 0.19      & 0.93    & 0.06 \\     
Ca I  & 10  & 3.32    & 0.14      & $-$3.02 & 0.11      & 0.27    & 0.07 \\     
Sc II & 8   & 0.09    & 0.14      & $-$3.06 & 0.09      & 0.21    & 0.07 \\     
Ti I  & 7   & 1.89    & 0.15      & $-$3.06 & 0.16      & 0.23    & 0.08 \\     
Ti II & 21  & 1.94    & 0.21      & $-$3.01 & 0.11      & 0.27    & 0.09 \\     
V I   & 2   & 0.62    & 0.03      & $-$3.31 & 0.12      & $-$0.02 & 0.11 \\     
V II  & 1   & 0.85    & 0.00      & $-$3.08 & 0.07      & 0.20    & 0.08 \\     
Cr I  & 4   & 1.87    & 0.20      & $-$3.78 & 0.19      & $-$0.49 & 0.11 \\     
Cr II & 1   & 2.51    & 0.00      & $-$3.13 & 0.07      & 0.15    & 0.05 \\     
Fe I  & 130 & 4.21    & 0.27      & $-$3.29 & 0.15      & 0.00    & 0.00 \\     
Fe II & 14  & 4.22    & 0.17      & $-$3.28 & 0.08      & 0.00    & 0.00 \\     
Co I  & 4   & 1.86    & 0.13      & $-$3.14 & 0.17      & 0.15    & 0.09 \\     
Ni I  & 3   & 3.30    & 0.05      & $-$2.92 & 0.16      & 0.37    & 0.06 \\     
Sr II & 2   & $-$0.48 & 0.08      & $-$3.35 & 0.36      & $-$0.07 & 0.34 \\     
Ba II & 4   & $-$2.16 & 0.15      & $-$4.34 & 0.11      & $-$1.06 & 0.11 \\     
C$-$H & 2   & 4.73    & 0.05      & $-$3.70 & 0.26      & $-$0.41 & 0.19 \\     
Mn I  & 1   & 1.94    & $\nodata$ & $-$3.49 & $\nodata$ & $-$0.20 & $\nodata$ \\
Y II  & 2   & $-$0.96 & $\nodata$ & $-$3.17 & $\nodata$ & 0.11    & $\nodata$ \\
Zr II & 1   & $-$0.38 & $\nodata$ & $-$2.96 & $\nodata$ & 0.31    & $\nodata$ \\
La II & 3   & $-$1.82 & $\nodata$ & $-$2.92 & $\nodata$ & 0.36    & $\nodata$ \\
Eu II & 2   & $-$2.38 & $\nodata$ & $-$2.90 & $\nodata$ & 0.37    & $\nodata$ \\
Dy II & 2   & $-$1.43 & $\nodata$ & $-$2.53 & $\nodata$ & 0.75    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr452} \\ \hline
Na I  & 2   & 3.78    & 0.16      & $-$2.46 & 0.29      & 0.69    & 0.17 \\     
Mg I  & 5   & 4.83    & 0.15      & $-$2.77 & 0.15      & 0.38    & 0.08 \\     
Al I  & 2   & 2.83    & 0.04      & $-$3.62 & 0.22      & $-$0.47 & 0.08 \\     
Si I  & 2   & 5.13    & 0.13      & $-$2.38 & 0.22      & 0.78    & 0.10 \\     
Ca I  & 12  & 3.42    & 0.20      & $-$2.92 & 0.13      & 0.23    & 0.08 \\     
Sc II & 8   & 0.09    & 0.15      & $-$3.06 & 0.09      & 0.10    & 0.07 \\     
Ti I  & 9   & 1.82    & 0.16      & $-$3.14 & 0.18      & 0.02    & 0.07 \\     
Ti II & 23  & 1.96    & 0.15      & $-$2.99 & 0.10      & 0.17    & 0.08 \\     
V I   & 2   & 0.48    & 0.02      & $-$3.45 & 0.13      & $-$0.30 & 0.10 \\     
V II  & 1   & 0.86    & 0.00      & $-$3.07 & 0.09      & 0.09    & 0.08 \\     
Cr I  & 4   & 1.86    & 0.23      & $-$3.78 & 0.23      & $-$0.62 & 0.12 \\     
Mn I  & 3   & 1.82    & 0.14      & $-$3.61 & 0.14      & $-$0.46 & 0.11 \\     
Fe I  & 117 & 4.34    & 0.21      & $-$3.16 & 0.17      & 0.00    & 0.00 \\     
Fe II & 14  & 4.34    & 0.12      & $-$3.16 & 0.07      & 0.00    & 0.00 \\     
Co I  & 4   & 1.79    & 0.24      & $-$3.20 & 0.19      & $-$0.05 & 0.13 \\     
Ni I  & 4   & 2.84    & 0.35      & $-$3.38 & 0.24      & $-$0.23 & 0.18 \\     
Sr II & 2   & $-$0.99 & 0.00      & $-$3.86 & 0.24      & $-$0.70 & 0.21 \\     
Zr II & 1   & $-$0.58 & 0.00      & $-$3.16 & 0.07      & 0.00    & 0.04 \\     
Ba II & 4   & $-$2.40 & 0.06      & $-$4.58 & 0.08      & $-$1.42 & 0.07 \\     
C$-$H & 2   & 4.72    & 0.04      & $-$3.71 & 0.27      & $-$0.55 & 0.15 \\     
Zn I  & 1   & 2.40    & $\nodata$ & $-$2.17 & $\nodata$ & 0.99    & $\nodata$ \\
Y II  & 1   & $-$1.21 & $\nodata$ & $-$3.42 & $\nodata$ & $-$0.26 & $\nodata$ \\
La II & 1   & $-$1.49 & $\nodata$ & $-$2.59 & $\nodata$ & 0.57    & $\nodata$ \\
Eu II & 2   & $-$2.49 & $\nodata$ & $-$3.01 & $\nodata$ & 0.15    & $\nodata$ \\
Dy II & 1   & $-$1.00 & $\nodata$ & $-$2.10 & $\nodata$ & 1.06    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr442} \\ \hline
Na I  & 2   & 3.99    & 0.00      & $-$2.25 & 0.27      & 0.96    & 0.14 \\     
Mg I  & 5   & 4.58    & 0.13      & $-$3.02 & 0.14      & 0.19    & 0.07 \\     
Al I  & 2   & 2.38    & 0.22      & $-$4.07 & 0.23      & $-$0.87 & 0.18 \\     
Si I  & 2   & 4.96    & 0.02      & $-$2.55 & 0.18      & 0.66    & 0.07 \\     
Ca I  & 14  & 3.54    & 0.17      & $-$2.80 & 0.12      & 0.41    & 0.07 \\     
Sc II & 8   & 0.12    & 0.09      & $-$3.03 & 0.07      & 0.14    & 0.06 \\     
Ti I  & 9   & 1.84    & 0.24      & $-$3.12 & 0.18      & 0.09    & 0.09 \\     
Ti II & 22  & 1.96    & 0.15      & $-$2.99 & 0.10      & 0.18    & 0.08 \\     
V I   & 2   & 0.69    & 0.07      & $-$3.24 & 0.13      & $-$0.04 & 0.11 \\     
V II  & 2   & 0.89    & 0.03      & $-$3.04 & 0.07      & 0.13    & 0.08 \\     
Cr I  & 4   & 1.89    & 0.25      & $-$3.75 & 0.22      & $-$0.54 & 0.13 \\     
Mn I  & 6   & 1.53    & 0.15      & $-$3.91 & 0.11      & $-$0.70 & 0.10 \\     
Fe I  & 139 & 4.29    & 0.26      & $-$3.21 & 0.16      & 0.00    & 0.00 \\     
Fe II & 15  & 4.33    & 0.17      & $-$3.17 & 0.07      & 0.00    & 0.00 \\     
Co I  & 4   & 2.09    & 0.24      & $-$2.90 & 0.14      & 0.31    & 0.15 \\     
Ni I  & 1   & 2.89    & 0.00      & $-$3.34 & 0.16      & $-$0.13 & 0.04 \\     
Zn I  & 1   & 1.62    & 0.00      & $-$2.94 & 0.05      & 0.27    & 0.12 \\     
Sr II & 2   & 0.45    & 0.01      & $-$2.42 & 0.24      & 0.75    & 0.23 \\     
Y II  & 3   & $-$0.78 & 0.06      & $-$2.99 & 0.07      & 0.19    & 0.07 \\     
Zr II & 1   & $-$0.24 & 0.00      & $-$2.82 & 0.07      & 0.36    & 0.06 \\     
Ba II & 5   & $-$1.90 & 0.23      & $-$4.08 & 0.13      & $-$0.91 & 0.13 \\     
C$-$H & 2   & 4.82    & 0.06      & $-$3.61 & 0.27      & $-$0.40 & 0.19 \\     
La II & 3   & $-$1.85 & $\nodata$ & $-$2.95 & $\nodata$ & 0.23    & $\nodata$ \\
Eu II & 2   & $-$2.67 & $\nodata$ & $-$3.19 & $\nodata$ & $-$0.01 & $\nodata$ \\
Dy II & 2   & $-$1.60 & $\nodata$ & $-$2.70 & $\nodata$ & 0.48    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr460} \\ \hline
Na I  & 2   & 3.91    & 0.10      & $-$2.33 & 0.25      & 0.67    & 0.14 \\     
Mg I  & 5   & 4.98    & 0.11      & $-$2.62 & 0.14      & 0.38    & 0.07 \\     
Al I  & 2   & 2.95    & 0.32      & $-$3.51 & 0.26      & $-$0.51 & 0.25 \\     
Si I  & 2   & 5.11    & 0.02      & $-$2.40 & 0.17      & 0.60    & 0.04 \\     
Ca I  & 12  & 3.63    & 0.19      & $-$2.71 & 0.12      & 0.29    & 0.07 \\     
Sc II & 8   & 0.28    & 0.10      & $-$2.87 & 0.08      & 0.07    & 0.05 \\     
Ti I  & 10  & 2.15    & 0.13      & $-$2.80 & 0.17      & 0.20    & 0.06 \\     
Ti II & 24  & 2.29    & 0.14      & $-$2.66 & 0.11      & 0.27    & 0.08 \\     
V II  & 2   & 1.06    & 0.13      & $-$2.87 & 0.11      & 0.06    & 0.12 \\     
Cr I  & 6   & 2.37    & 0.18      & $-$3.27 & 0.19      & $-$0.27 & 0.08 \\     
Cr II & 1   & 2.81    & 0.00      & $-$2.83 & 0.07      & 0.11    & 0.04 \\     
Mn I  & 6   & 2.09    & 0.15      & $-$3.34 & 0.12      & $-$0.34 & 0.09 \\     
Fe I  & 138 & 4.50    & 0.24      & $-$3.00 & 0.16      & 0.00    & 0.00 \\     
Fe II & 14  & 4.56    & 0.11      & $-$2.94 & 0.07      & 0.00    & 0.00 \\     
Co I  & 4   & 2.06    & 0.11      & $-$2.94 & 0.14      & 0.06    & 0.07 \\     
Ni I  & 4   & 3.29    & 0.20      & $-$2.93 & 0.20      & 0.07    & 0.11 \\     
Sr II & 2   & $-$0.05 & 0.01      & $-$2.92 & 0.30      & 0.02    & 0.28 \\     
Zr II & 1   & $-$0.31 & 0.00      & $-$2.89 & 0.06      & 0.05    & 0.04 \\     
Ba II & 5   & $-$1.83 & 0.12      & $-$4.01 & 0.10      & $-$1.07 & 0.09 \\     
C$-$H & 2   & 4.66    & 0.13      & $-$3.77 & 0.25      & $-$0.77 & 0.19 \\     
C$-$N & 1   & 5.89    & 0.00      & $-$1.94 & 0.33      & 1.06    & 0.28 \\     
Zn I  & 1   & 2.08    & $\nodata$ & $-$2.48 & $\nodata$ & 0.52    & $\nodata$ \\
Y II  & 3   & $-$0.97 & $\nodata$ & $-$3.18 & $\nodata$ & $-$0.24 & $\nodata$ \\
La II & 3   & $-$1.62 & $\nodata$ & $-$2.72 & $\nodata$ & 0.22    & $\nodata$ \\
Eu II & 2   & $-$2.26 & $\nodata$ & $-$2.78 & $\nodata$ & 0.16    & $\nodata$ \\
Dy II & 2   & $-$1.48 & $\nodata$ & $-$2.58 & $\nodata$ & 0.36    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr484} \\ \hline
Na I  & 2   & 4.17    & 0.04      & $-$2.08 & 0.24      & 0.87    & 0.13 \\     
Mg I  & 5   & 5.01    & 0.10      & $-$2.59 & 0.14      & 0.35    & 0.06 \\     
Al I  & 2   & 3.36    & 0.03      & $-$3.09 & 0.21      & $-$0.15 & 0.08 \\     
Si I  & 2   & 5.23    & 0.01      & $-$2.28 & 0.19      & 0.66    & 0.05 \\     
Ca I  & 12  & 3.57    & 0.16      & $-$2.78 & 0.12      & 0.17    & 0.07 \\     
Sc II & 8   & 0.19    & 0.09      & $-$2.96 & 0.10      & 0.02    & 0.06 \\     
Ti I  & 10  & 2.09    & 0.10      & $-$2.86 & 0.17      & 0.09    & 0.06 \\     
Ti II & 25  & 2.27    & 0.10      & $-$2.68 & 0.13      & 0.30    & 0.08 \\     
V I   & 2   & 0.87    & 0.00      & $-$3.06 & 0.14      & $-$0.12 & 0.11 \\     
V II  & 1   & 0.90    & 0.00      & $-$3.03 & 0.14      & $-$0.05 & 0.14 \\     
Cr I  & 6   & 2.30    & 0.16      & $-$3.34 & 0.19      & $-$0.40 & 0.08 \\     
Mn I  & 3   & 2.10    & 0.09      & $-$3.33 & 0.13      & $-$0.39 & 0.08 \\     
Fe I  & 153 & 4.56    & 0.26      & $-$2.94 & 0.15      & 0.00    & 0.00 \\     
Fe II & 14  & 4.52    & 0.16      & $-$2.98 & 0.09      & 0.00    & 0.00 \\     
Co I  & 4   & 2.27    & 0.23      & $-$2.72 & 0.17      & 0.22    & 0.13 \\     
Ni I  & 5   & 3.24    & 0.15      & $-$2.98 & 0.18      & $-$0.04 & 0.07 \\     
Zn I  & 1   & 1.99    & 0.00      & $-$2.58 & 0.07      & 0.37    & 0.10 \\     
Sr II & 2   & $-$0.20 & 0.03      & $-$3.07 & 0.32      & $-$0.09 & 0.29 \\     
Y II  & 1   & $-$1.09 & 0.00      & $-$3.30 & 0.10      & $-$0.32 & 0.09 \\     
Zr II & 1   & $-$0.26 & 0.00      & $-$2.84 & 0.09      & 0.14    & 0.07 \\     
Ba II & 5   & $-$1.72 & 0.24      & $-$3.90 & 0.15      & $-$0.92 & 0.13 \\     
C$-$H & 2   & 5.08    & 0.03      & $-$3.35 & 0.31      & $-$0.41 & 0.20 \\     
La II & 3   & $-$1.68 & $\nodata$ & $-$2.78 & $\nodata$ & 0.20    & $\nodata$ \\
Eu II & 3   & $-$2.48 & $\nodata$ & $-$3.00 & $\nodata$ & $-$0.02 & $\nodata$ \\
Dy II & 2   & $-$1.58 & $\nodata$ & $-$2.68 & $\nodata$ & 0.30    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr482} \\ \hline
Na I  & 2   & 4.22    & 0.00      & $-$2.02 & 0.25      & 0.71    & 0.10 \\     
Mg I  & 4   & 5.23    & 0.07      & $-$2.38 & 0.16      & 0.36    & 0.05 \\     
Al I  & 1   & 3.39    & 0.00      & $-$3.06 & 0.20      & $-$0.32 & 0.20 \\     
Si I  & 2   & 5.25    & 0.07      & $-$2.26 & 0.21      & 0.47    & 0.07 \\     
Ca I  & 17  & 3.93    & 0.15      & $-$2.41 & 0.12      & 0.33    & 0.07 \\     
Sc II & 8   & 0.40    & 0.13      & $-$2.75 & 0.12      & $-$0.03 & 0.08 \\     
Ti I  & 16  & 2.30    & 0.21      & $-$2.65 & 0.19      & 0.09    & 0.07 \\     
Ti II & 26  & 2.51    & 0.19      & $-$2.44 & 0.13      & 0.28    & 0.08 \\     
V I   & 2   & 1.10    & 0.16      & $-$2.83 & 0.12      & $-$0.10 & 0.20 \\     
V II  & 2   & 1.17    & 0.03      & $-$2.77 & 0.15      & $-$0.04 & 0.12 \\     
Cr I  & 7   & 2.68    & 0.15      & $-$2.96 & 0.18      & $-$0.23 & 0.07 \\     
Cr II & 2   & 3.05    & 0.11      & $-$2.59 & 0.11      & 0.14    & 0.10 \\     
Mn I  & 6   & 2.11    & 0.07      & $-$3.32 & 0.11      & $-$0.58 & 0.09 \\     
Fe I  & 160 & 4.76    & 0.19      & $-$2.74 & 0.17      & 0.00    & 0.00 \\     
Fe II & 13  & 4.78    & 0.13      & $-$2.72 & 0.10      & 0.00    & 0.00 \\     
Co I  & 4   & 2.34    & 0.25      & $-$2.65 & 0.19      & 0.08    & 0.13 \\     
Ni I  & 7   & 3.56    & 0.19      & $-$2.66 & 0.15      & 0.08    & 0.09 \\     
Zn I  & 1   & 1.88    & 0.00      & $-$2.68 & 0.05      & 0.06    & 0.15 \\     
Sr II & 2   & 0.43    & 0.02      & $-$2.44 & 0.18      & 0.28    & 0.14 \\     
Y II  & 3   & $-$0.42 & 0.07      & $-$2.63 & 0.10      & 0.10    & 0.07 \\     
Zr II & 1   & 0.20    & 0.00      & $-$2.38 & 0.09      & 0.34    & 0.05 \\     
Ba II & 5   & $-$0.42 & 0.07      & $-$2.60 & 0.17      & 0.12    & 0.12 \\     
La II & 2   & $-$1.78 & 0.03      & $-$2.88 & 0.09      & $-$0.16 & 0.09 \\     
C$-$H & 2   & 5.89    & 0.01      & $-$2.54 & 0.29      & 0.19    & 0.17 \\     
C$-$N & 1   & 6.13    & 0.00      & $-$1.70 & 0.39      & 1.04    & 0.25 \\     
Eu II & 3   & $-$2.22 & $\nodata$ & $-$2.74 & $\nodata$ & $-$0.02 & $\nodata$ \\
Dy II & 2   & $-$1.64 & $\nodata$ & $-$2.74 & $\nodata$ & $-$0.02 & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr495} \\ \hline
Na I  & 2   & 3.49    & 0.02      & $-$2.75 & 0.27      & 0.21    & 0.13 \\     
Mg I  & 5   & 5.12    & 0.12      & $-$2.48 & 0.16      & 0.48    & 0.07 \\     
Al I  & 2   & 2.99    & 0.07      & $-$3.46 & 0.26      & $-$0.50 & 0.16 \\     
Si I  & 2   & 4.87    & 0.24      & $-$2.64 & 0.30      & 0.31    & 0.19 \\     
Ca I  & 14  & 3.53    & 0.16      & $-$2.81 & 0.13      & 0.15    & 0.07 \\     
Sc II & 8   & 0.15    & 0.19      & $-$3.00 & 0.13      & $-$0.08 & 0.08 \\     
Ti I  & 16  & 2.09    & 0.15      & $-$2.86 & 0.21      & 0.10    & 0.06 \\     
Ti II & 28  & 2.25    & 0.13      & $-$2.70 & 0.13      & 0.23    & 0.08 \\     
V I   & 2   & 0.74    & 0.06      & $-$3.19 & 0.15      & $-$0.23 & 0.10 \\     
V II  & 2   & 0.91    & 0.05      & $-$3.02 & 0.15      & $-$0.10 & 0.10 \\     
Cr I  & 7   & 2.32    & 0.16      & $-$3.32 & 0.20      & $-$0.36 & 0.07 \\     
Cr II & 1   & 2.62    & 0.00      & $-$3.02 & 0.10      & $-$0.10 & 0.05 \\     
Mn I  & 6   & 2.01    & 0.17      & $-$3.42 & 0.13      & $-$0.46 & 0.10 \\     
Fe I  & 164 & 4.54    & 0.22      & $-$2.96 & 0.17      & 0.00    & 0.00 \\     
Fe II & 16  & 4.57    & 0.16      & $-$2.93 & 0.11      & 0.00    & 0.00 \\     
Co I  & 4   & 2.15    & 0.29      & $-$2.84 & 0.22      & 0.12    & 0.15 \\     
Ni I  & 5   & 3.34    & 0.18      & $-$2.88 & 0.18      & 0.08    & 0.09 \\     
Zn I  & 1   & 1.72    & 0.00      & $-$2.84 & 0.07      & 0.12    & 0.17 \\     
Sr II & 2   & $-$0.14 & 0.02      & $-$3.01 & 0.23      & $-$0.08 & 0.19 \\     
Y II  & 3   & $-$1.09 & 0.15      & $-$3.30 & 0.16      & $-$0.37 & 0.12 \\     
Zr II & 1   & $-$0.29 & 0.00      & $-$2.87 & 0.11      & 0.06    & 0.05 \\     
Ba II & 5   & $-$1.46 & 0.09      & $-$3.64 & 0.14      & $-$0.71 & 0.09 \\     
Eu II & 2   & $-$2.53 & 0.05      & $-$3.05 & 0.16      & $-$0.12 & 0.11 \\     
Dy II & 2   & $-$1.66 & 0.04      & $-$2.76 & 0.18      & 0.16    & 0.10 \\     
C$-$H & 2   & 4.96    & 0.05      & $-$3.47 & 0.32      & $-$0.51 & 0.20 \\     
C$-$N & 1   & 5.49    & 0.00      & $-$2.34 & 0.36      & 0.62    & 0.26 \\     
La II & 3   & $-$2.00 & $\nodata$ & $-$3.10 & $\nodata$ & $-$0.17 & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr496} \\ \hline
Na I  & 2   & 4.16    & 0.04      & $-$2.08 & 0.26      & 0.87    & 0.11 \\     
Mg I  & 5   & 5.05    & 0.13      & $-$2.55 & 0.15      & 0.40    & 0.08 \\     
Al I  & 2   & 3.50    & 0.15      & $-$2.95 & 0.29      & 0.00    & 0.17 \\     
Si I  & 2   & 5.08    & 0.12      & $-$2.43 & 0.21      & 0.52    & 0.10 \\     
Ca I  & 16  & 3.69    & 0.27      & $-$2.65 & 0.14      & 0.30    & 0.10 \\     
Sc II & 8   & 0.26    & 0.15      & $-$2.89 & 0.11      & 0.13    & 0.08 \\     
Ti I  & 12  & 2.03    & 0.22      & $-$2.92 & 0.20      & 0.03    & 0.09 \\     
Ti II & 24  & 2.33    & 0.12      & $-$2.62 & 0.13      & 0.39    & 0.09 \\     
V I   & 2   & 0.64    & 0.03      & $-$3.29 & 0.14      & $-$0.34 & 0.12 \\     
V II  & 2   & 1.17    & 0.09      & $-$2.77 & 0.15      & 0.25    & 0.12 \\     
Cr I  & 5   & 2.30    & 0.16      & $-$3.34 & 0.22      & $-$0.39 & 0.08 \\     
Mn I  & 5   & 1.98    & 0.16      & $-$3.45 & 0.13      & $-$0.50 & 0.12 \\     
Fe I  & 148 & 4.55    & 0.26      & $-$2.95 & 0.18      & 0.00    & 0.00 \\     
Fe II & 15  & 4.49    & 0.16      & $-$3.01 & 0.09      & 0.00    & 0.00 \\     
Co I  & 4   & 2.25    & 0.18      & $-$2.74 & 0.17      & 0.21    & 0.10 \\     
Ni I  & 5   & 3.33    & 0.10      & $-$2.89 & 0.20      & 0.07    & 0.05 \\     
Zn I  & 1   & 1.80    & 0.00      & $-$2.76 & 0.05      & 0.19    & 0.14 \\     
Sr II & 2   & 0.08    & 0.00      & $-$2.79 & 0.29      & 0.22    & 0.26 \\     
Y II  & 2   & $-$1.09 & 0.14      & $-$3.30 & 0.12      & $-$0.29 & 0.13 \\     
Ba II & 5   & $-$1.86 & 0.07      & $-$4.04 & 0.07      & $-$1.03 & 0.08 \\     
C$-$H & 2   & 5.02    & 0.06      & $-$3.41 & 0.27      & $-$0.46 & 0.17 \\     
Zr II & 1   & $-$0.14 & $\nodata$ & $-$2.72 & $\nodata$ & 0.30    & $\nodata$ \\
La II & 3   & $-$1.76 & $\nodata$ & $-$2.86 & $\nodata$ & 0.15    & $\nodata$ \\
Eu II & 3   & $-$2.34 & $\nodata$ & $-$2.86 & $\nodata$ & 0.15    & $\nodata$ \\
Dy II & 2   & $-$1.42 & $\nodata$ & $-$2.52 & $\nodata$ & 0.50    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr509} \\ \hline
Na I  & 2   & 3.34    & 0.11      & $-$2.90 & 0.25      & 0.28    & 0.13 \\     
Mg I  & 5   & 4.71    & 0.10      & $-$2.89 & 0.14      & 0.29    & 0.07 \\     
Al I  & 2   & 2.58    & 0.04      & $-$3.87 & 0.20      & $-$0.69 & 0.10 \\     
Si I  & 2   & 4.82    & 0.05      & $-$2.69 & 0.25      & 0.50    & 0.18 \\     
Ca I  & 13  & 3.53    & 0.19      & $-$2.81 & 0.12      & 0.37    & 0.08 \\     
Sc II & 8   & 0.06    & 0.08      & $-$3.09 & 0.08      & 0.10    & 0.05 \\     
Ti I  & 10  & 1.87    & 0.14      & $-$3.08 & 0.17      & 0.11    & 0.07 \\     
Ti II & 22  & 2.04    & 0.15      & $-$2.91 & 0.11      & 0.28    & 0.08 \\     
V I   & 2   & 0.74    & 0.06      & $-$3.19 & 0.13      & $-$0.00 & 0.11 \\     
V II  & 2   & 0.76    & 0.01      & $-$3.18 & 0.08      & 0.02    & 0.07 \\     
Cr I  & 4   & 1.98    & 0.19      & $-$3.66 & 0.21      & $-$0.48 & 0.10 \\     
Mn I  & 2   & 2.07    & 0.03      & $-$3.36 & 0.10      & $-$0.18 & 0.08 \\     
Fe I  & 133 & 4.32    & 0.27      & $-$3.18 & 0.16      & 0.00    & 0.00 \\     
Fe II & 14  & 4.31    & 0.15      & $-$3.20 & 0.08      & 0.00    & 0.00 \\     
Co I  & 4   & 2.08    & 0.17      & $-$2.91 & 0.12      & 0.27    & 0.12 \\     
Ni I  & 2   & 3.07    & 0.10      & $-$3.15 & 0.25      & 0.03    & 0.13 \\     
Zn I  & 1   & 1.79    & 0.00      & $-$2.77 & 0.06      & 0.41    & 0.12 \\     
Sr II & 2   & $-$0.27 & 0.12      & $-$3.14 & 0.34      & 0.05    & 0.32 \\     
Y II  & 2   & $-$0.95 & 0.04      & $-$3.16 & 0.08      & 0.03    & 0.07 \\     
Zr II & 1   & $-$0.10 & 0.00      & $-$2.68 & 0.08      & 0.52    & 0.04 \\     
Ba II & 4   & $-$1.98 & 0.11      & $-$4.16 & 0.09      & $-$0.97 & 0.08 \\     
C$-$H & 2   & 5.04    & 0.06      & $-$3.39 & 0.27      & $-$0.20 & 0.17 \\     
La II & 2   & $-$1.83 & $\nodata$ & $-$2.93 & $\nodata$ & 0.27    & $\nodata$ \\
Eu II & 3   & $-$2.35 & $\nodata$ & $-$2.87 & $\nodata$ & 0.33    & $\nodata$ \\
Dy II & 1   & $-$1.49 & $\nodata$ & $-$2.59 & $\nodata$ & 0.61    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr512} \\ \hline
Na I  & 2   & 3.43    & 0.11      & $-$2.81 & 0.24      & 0.21    & 0.15 \\     
Mg I  & 4   & 4.84    & 0.14      & $-$2.76 & 0.16      & 0.26    & 0.08 \\     
Al I  & 2   & 3.04    & 0.02      & $-$3.41 & 0.25      & $-$0.38 & 0.13 \\     
Si I  & 2   & 5.11    & 0.25      & $-$2.40 & 0.28      & 0.63    & 0.19 \\     
Ca I  & 13  & 3.53    & 0.16      & $-$2.81 & 0.12      & 0.22    & 0.07 \\     
Sc II & 8   & 0.06    & 0.13      & $-$3.09 & 0.10      & 0.05    & 0.07 \\     
Ti I  & 14  & 2.08    & 0.22      & $-$2.87 & 0.18      & 0.16    & 0.08 \\     
Ti II & 24  & 2.21    & 0.15      & $-$2.74 & 0.13      & 0.41    & 0.09 \\     
V II  & 1   & 0.89    & 0.00      & $-$3.04 & 0.08      & 0.10    & 0.06 \\     
Cr I  & 4   & 2.14    & 0.20      & $-$3.50 & 0.22      & $-$0.47 & 0.12 \\     
Mn I  & 2   & 1.63    & 0.08      & $-$3.80 & 0.12      & $-$0.77 & 0.10 \\     
Fe I  & 144 & 4.47    & 0.27      & $-$3.03 & 0.16      & 0.00    & 0.00 \\     
Fe II & 14  & 4.35    & 0.13      & $-$3.15 & 0.09      & 0.00    & 0.00 \\     
Co I  & 4   & 1.99    & 0.22      & $-$3.00 & 0.18      & 0.02    & 0.12 \\     
Ni I  & 3   & 3.12    & 0.17      & $-$3.10 & 0.22      & $-$0.07 & 0.12 \\     
Zn I  & 1   & 2.02    & 0.00      & $-$2.54 & 0.07      & 0.49    & 0.11 \\     
Sr II & 2   & $-$0.40 & 0.24      & $-$3.27 & 0.35      & $-$0.13 & 0.32 \\     
Y II  & 2   & $-$1.10 & 0.22      & $-$3.31 & 0.18      & $-$0.17 & 0.17 \\     
Ba II & 4   & $-$1.95 & 0.05      & $-$4.13 & 0.11      & $-$0.99 & 0.09 \\     
C$-$H & 2   & 4.96    & 0.01      & $-$3.47 & 0.32      & $-$0.45 & 0.21 \\     
V I   & 1   & 0.94    & $\nodata$ & $-$2.99 & $\nodata$ & 0.04    & $\nodata$ \\
Zr II & 1   & $-$0.06 & $\nodata$ & $-$2.64 & $\nodata$ & 0.51    & $\nodata$ \\
La II & 1   & $-$1.44 & $\nodata$ & $-$2.54 & $\nodata$ & 0.61    & $\nodata$ \\
Eu II & 3   & $-$2.36 & $\nodata$ & $-$2.88 & $\nodata$ & 0.27    & $\nodata$ \\
Dy II & 2   & $-$1.43 & $\nodata$ & $-$2.53 & $\nodata$ & 0.62    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr422} \\ \hline
Na I  & 2   & 4.54    & 0.01 & $-$1.70 & 0.23 & 0.24    & 0.07 \\
Mg I  & 5   & 5.76    & 0.24 & $-$1.84 & 0.19 & 0.10    & 0.13 \\
Al I  & 2   & 3.73    & 0.03 & $-$2.72 & 0.26 & $-$0.79 & 0.12 \\
Si I  & 2   & 5.86    & 0.11 & $-$1.66 & 0.21 & 0.28    & 0.09 \\
Ca I  & 17  & 4.65    & 0.24 & $-$1.69 & 0.15 & 0.25    & 0.08 \\
Sc II & 8   & 1.37    & 0.21 & $-$1.78 & 0.15 & $-$0.04 & 0.10 \\
Ti I  & 10  & 3.22    & 0.26 & $-$1.73 & 0.20 & 0.20    & 0.09 \\
Ti II & 28  & 3.53    & 0.25 & $-$1.42 & 0.18 & 0.32    & 0.10 \\
V I   & 2   & 1.67    & 0.09 & $-$2.26 & 0.15 & $-$0.33 & 0.16 \\
V II  & 2   & 2.39    & 0.28 & $-$1.54 & 0.20 & 0.20    & 0.24 \\
Cr I  & 6   & 3.51    & 0.16 & $-$2.13 & 0.24 & $-$0.19 & 0.08 \\
Cr II & 3   & 3.88    & 0.11 & $-$1.76 & 0.11 & $-$0.02 & 0.12 \\
Mn I  & 6   & 3.06    & 0.22 & $-$2.37 & 0.12 & $-$0.43 & 0.16 \\
Fe I  & 146 & 5.57    & 0.28 & $-$1.93 & 0.19 & 0.00    & 0.00 \\
Fe II & 13  & 5.76    & 0.24 & $-$1.74 & 0.16 & 0.00    & 0.00 \\
Co I  & 4   & 3.18    & 0.37 & $-$1.81 & 0.23 & 0.12    & 0.20 \\
Ni I  & 4   & 4.37    & 0.12 & $-$1.85 & 0.14 & 0.09    & 0.11 \\
Zn I  & 1   & 2.76    & 0.00 & $-$1.80 & 0.06 & 0.13    & 0.16 \\
Sr II & 2   & 1.02    & 0.00 & $-$1.85 & 0.14 & $-$0.10 & 0.11 \\
Y II  & 3   & 0.17    & 0.10 & $-$2.04 & 0.11 & $-$0.30 & 0.12 \\
Zr II & 1   & 0.92    & 0.00 & $-$1.66 & 0.08 & 0.09    & 0.13 \\
Ba II & 5   & 0.56    & 0.27 & $-$1.62 & 0.24 & 0.12    & 0.17 \\
La II & 2   & $-$0.62 & 0.06 & $-$1.72 & 0.09 & 0.02    & 0.14 \\
Eu II & 2   & $-$0.79 & 0.07 & $-$1.31 & 0.10 & 0.43    & 0.16 \\
Dy II & 2   & $-$0.32 & 0.13 & $-$1.42 & 0.13 & 0.33    & 0.17 \\
C$-$H & 2   & 5.88    & 0.00 & $-$2.55 & 0.23 & $-$0.62 & 0.20 \\
C$-$N & 1   & 6.53    & 0.00 & $-$1.30 & 0.30 & 0.64    & 0.24 \\
\hline \multicolumn{8}{c}{Sgr424} \\ \hline
Na I  & 2   & 4.09    & 0.05      & $-$2.15 & 0.25      & 0.28    & 0.10 \\     
Mg I  & 5   & 5.47    & 0.15      & $-$2.13 & 0.16      & 0.31    & 0.09 \\     
Al I  & 1   & 3.68    & 0.00      & $-$2.77 & 0.17      & $-$0.34 & 0.11 \\     
Si I  & 2   & 5.48    & 0.11      & $-$2.03 & 0.24      & 0.40    & 0.11 \\     
Ca I  & 13  & 4.21    & 0.12      & $-$2.13 & 0.12      & 0.30    & 0.07 \\     
Sc II & 7   & 0.77    & 0.13      & $-$2.38 & 0.12      & 0.11    & 0.08 \\     
Ti I  & 15  & 2.67    & 0.22      & $-$2.28 & 0.18      & 0.15    & 0.07 \\     
Ti II & 25  & 2.81    & 0.18      & $-$2.14 & 0.15      & 0.34    & 0.10 \\     
V I   & 3   & 1.52    & 0.05      & $-$2.41 & 0.17      & 0.03    & 0.09 \\     
V II  & 1   & 1.63    & 0.00      & $-$2.31 & 0.09      & 0.18    & 0.11 \\     
Cr I  & 6   & 2.86    & 0.12      & $-$2.78 & 0.17      & $-$0.34 & 0.07 \\     
Cr II & 2   & 2.99    & 0.09      & $-$2.65 & 0.10      & $-$0.17 & 0.10 \\     
Mn I  & 6   & 2.58    & 0.06      & $-$2.85 & 0.09      & $-$0.42 & 0.11 \\     
Fe I  & 162 & 5.07    & 0.23      & $-$2.43 & 0.17      & 0.00    & 0.00 \\     
Fe II & 15  & 5.02    & 0.21      & $-$2.48 & 0.11      & 0.00    & 0.00 \\     
Co I  & 4   & 2.77    & 0.02      & $-$2.22 & 0.12      & 0.22    & 0.07 \\     
Ni I  & 6   & 3.87    & 0.16      & $-$2.35 & 0.15      & 0.08    & 0.08 \\     
Zn I  & 1   & 2.19    & 0.00      & $-$2.37 & 0.05      & 0.06    & 0.14 \\     
Sr II & 2   & 0.08    & 0.31      & $-$2.79 & 0.31      & $-$0.31 & 0.27 \\     
Y II  & 2   & $-$0.69 & 0.03      & $-$2.90 & 0.08      & $-$0.42 & 0.09 \\     
Ba II & 5   & $-$1.05 & 0.11      & $-$3.23 & 0.12      & $-$0.75 & 0.10 \\     
Eu II & 2   & $-$1.93 & 0.13      & $-$2.45 & 0.13      & 0.03    & 0.13 \\     
C$-$H & 2   & 5.93    & 0.02      & $-$2.50 & 0.28      & $-$0.07 & 0.18 \\     
C$-$N & 1   & 5.81    & 0.00      & $-$2.02 & 0.32      & 0.42    & 0.24 \\     
Zr II & 1   & 0.23    & $\nodata$ & $-$2.35 & $\nodata$ & 0.14    & $\nodata$ \\
La II & 3   & $-$1.22 & $\nodata$ & $-$2.32 & $\nodata$ & 0.16    & $\nodata$ \\
Dy II & 2   & $-$0.91 & $\nodata$ & $-$2.01 & $\nodata$ & 0.47    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr441} \\ \hline
Na I  & 2   & 3.93    & 0.03      & $-$2.31 & 0.35      & 0.47    & 0.16 \\     
Mg I  & 3   & 5.07    & 0.09      & $-$2.53 & 0.22      & 0.25    & 0.07 \\     
Al I  & 2   & 3.15    & 0.14      & $-$3.30 & 0.32      & $-$0.52 & 0.17 \\     
Si I  & 1   & 5.35    & 0.00      & $-$2.16 & 0.22      & 0.62    & 0.07 \\     
Ca I  & 21  & 3.91    & 0.28      & $-$2.43 & 0.15      & 0.35    & 0.09 \\     
Sc II & 8   & 0.39    & 0.16      & $-$2.76 & 0.12      & $-$0.09 & 0.07 \\     
Ti I  & 17  & 2.13    & 0.20      & $-$2.82 & 0.26      & $-$0.04 & 0.08 \\     
Ti II & 26  & 2.52    & 0.18      & $-$2.43 & 0.13      & 0.25    & 0.10 \\     
V I   & 2   & 0.76    & 0.05      & $-$3.17 & 0.20      & $-$0.39 & 0.09 \\     
V II  & 1   & 1.15    & 0.00      & $-$2.78 & 0.11      & $-$0.11 & 0.15 \\     
Cr I  & 8   & 2.54    & 0.24      & $-$3.10 & 0.29      & $-$0.32 & 0.11 \\     
Mn I  & 6   & 1.91    & 0.16      & $-$3.52 & 0.15      & $-$0.74 & 0.11 \\     
Fe I  & 164 & 4.72    & 0.23      & $-$2.78 & 0.21      & 0.00    & 0.00 \\     
Fe II & 14  & 4.83    & 0.16      & $-$2.67 & 0.10      & 0.00    & 0.00 \\     
Co I  & 4   & 2.21    & 0.19      & $-$2.78 & 0.23      & 0.00    & 0.10 \\     
Ni I  & 4   & 3.43    & 0.13      & $-$2.79 & 0.19      & $-$0.01 & 0.09 \\     
Zn I  & 1   & 1.48    & 0.00      & $-$3.08 & 0.04      & $-$0.30 & 0.19 \\     
Sr II & 2   & $-$0.50 & 0.03      & $-$3.37 & 0.18      & $-$0.70 & 0.12 \\     
Y II  & 1   & $-$1.24 & 0.00      & $-$3.45 & 0.07      & $-$0.77 & 0.07 \\     
Ba II & 5   & $-$1.32 & 0.05      & $-$3.50 & 0.09      & $-$0.83 & 0.09 \\     
La II & 2   & $-$1.85 & 0.18      & $-$2.95 & 0.15      & $-$0.28 & 0.17 \\     
Eu II & 2   & $-$2.73 & 0.06      & $-$3.25 & 0.09      & $-$0.58 & 0.11 \\     
C$-$H & 2   & 4.77    & 0.02      & $-$3.66 & 0.23      & $-$0.88 & 0.15 \\     
Zr II & 1   & $-$0.04 & $\nodata$ & $-$2.62 & $\nodata$ & 0.05    & $\nodata$ \\
Dy II & 2   & $-$1.42 & $\nodata$ & $-$2.52 & $\nodata$ & 0.15    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr438} \\ \hline
Na I  & 2   & 3.15    & 0.02      & $-$3.10 & 0.17      & $-$0.56 & 0.04 \\     
Mg I  & 4   & 4.85    & 0.15      & $-$2.75 & 0.15      & $-$0.21 & 0.10 \\     
Al I  & 2   & 2.46    & 0.01      & $-$4.00 & 0.24      & $-$1.46 & 0.11 \\     
Si I  & 2   & 4.99    & 0.07      & $-$2.52 & 0.19      & 0.02    & 0.08 \\     
Ca I  & 9   & 3.75    & 0.14      & $-$2.59 & 0.12      & $-$0.06 & 0.07 \\     
Sc II & 7   & 0.07    & 0.17      & $-$3.08 & 0.14      & $-$0.48 & 0.08 \\     
Ti I  & 5   & 2.34    & 0.15      & $-$2.61 & 0.17      & $-$0.08 & 0.08 \\     
Ti II & 13  & 2.35    & 0.19      & $-$2.61 & 0.18      & $-$0.01 & 0.09 \\     
Cr I  & 3   & 2.76    & 0.05      & $-$2.88 & 0.19      & $-$0.35 & 0.05 \\     
Mn I  & 4   & 2.31    & 0.19      & $-$3.12 & 0.14      & $-$0.58 & 0.12 \\     
Fe I  & 142 & 4.97    & 0.23      & $-$2.53 & 0.16      & 0.00    & 0.00 \\     
Fe II & 16  & 4.91    & 0.15      & $-$2.60 & 0.14      & 0.00    & 0.00 \\     
Co I  & 2   & 2.01    & 0.09      & $-$2.98 & 0.16      & $-$0.45 & 0.09 \\     
Ni I  & 1   & 3.42    & 0.00      & $-$2.81 & 0.28      & $-$0.27 & 0.15 \\     
Sr II & 2   & $-$0.28 & 0.05      & $-$3.15 & 0.30      & $-$0.56 & 0.24 \\     
Ba II & 2   & $-$1.25 & 0.04      & $-$3.43 & 0.16      & $-$0.84 & 0.09 \\     
C$-$H & 2   & 6.10    & 0.04      & $-$2.33 & 0.25      & 0.20    & 0.15 \\     
Zn I  & 1   & 2.33    & $\nodata$ & $-$2.23 & $\nodata$ & 0.31    & $\nodata$ \\
Y II  & 1   & $-$0.21 & $\nodata$ & $-$2.42 & $\nodata$ & 0.18    & $\nodata$ \\
Zr II & 1   & 0.35    & $\nodata$ & $-$2.23 & $\nodata$ & 0.37    & $\nodata$ \\
La II & 2   & $-$1.06 & $\nodata$ & $-$2.16 & $\nodata$ & 0.43    & $\nodata$ \\
Eu II & 3   & $-$1.52 & $\nodata$ & $-$2.04 & $\nodata$ & 0.56    & $\nodata$ \\
Dy II & 1   & $-$0.01 & $\nodata$ & $-$1.11 & $\nodata$ & 1.49    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr463} \\ \hline
Na I  & 2   & 3.69    & 0.02      & $-$2.55 & 0.31      & 0.15    & 0.12 \\     
Mg I  & 4   & 5.18    & 0.08      & $-$2.43 & 0.18      & 0.27    & 0.06 \\     
Al I  & 2   & 3.09    & 0.34      & $-$3.36 & 0.51      & $-$0.67 & 0.36 \\     
Si I  & 2   & 5.22    & 0.21      & $-$2.29 & 0.27      & 0.40    & 0.15 \\     
Ca I  & 18  & 4.04    & 0.17      & $-$2.30 & 0.13      & 0.39    & 0.08 \\     
Sc II & 7   & 0.38    & 0.11      & $-$2.77 & 0.09      & $-$0.09 & 0.06 \\     
Ti I  & 17  & 2.27    & 0.14      & $-$2.68 & 0.22      & 0.01    & 0.06 \\     
Ti II & 28  & 2.54    & 0.17      & $-$2.41 & 0.11      & 0.27    & 0.09 \\     
V I   & 3   & 0.90    & 0.01      & $-$3.03 & 0.25      & $-$0.34 & 0.11 \\     
V II  & 2   & 1.24    & 0.04      & $-$2.69 & 0.10      & $-$0.01 & 0.09 \\     
Cr I  & 10  & 2.65    & 0.15      & $-$3.00 & 0.21      & $-$0.30 & 0.06 \\     
Cr II & 2   & 3.05    & 0.13      & $-$2.59 & 0.12      & 0.09    & 0.11 \\     
Mn I  & 5   & 2.12    & 0.13      & $-$3.32 & 0.13      & $-$0.62 & 0.11 \\     
Fe I  & 175 & 4.81    & 0.18      & $-$2.69 & 0.19      & 0.00    & 0.00 \\     
Fe II & 16  & 4.82    & 0.18      & $-$2.68 & 0.09      & 0.00    & 0.00 \\     
Co I  & 4   & 2.32    & 0.19      & $-$2.67 & 0.19      & 0.03    & 0.10 \\     
Ni I  & 6   & 3.36    & 0.24      & $-$2.86 & 0.21      & $-$0.17 & 0.10 \\     
Zn I  & 1   & 1.80    & 0.00      & $-$2.76 & 0.03      & $-$0.06 & 0.18 \\     
Sr II & 2   & 0.41    & 0.01      & $-$2.46 & 0.13      & 0.23    & 0.12 \\     
Y II  & 3   & $-$0.69 & 0.07      & $-$2.90 & 0.07      & $-$0.22 & 0.09 \\     
Zr II & 1   & $-$0.01 & 0.00      & $-$2.59 & 0.08      & 0.09    & 0.07 \\     
Ba II & 5   & $-$1.10 & 0.10      & $-$3.28 & 0.09      & $-$0.60 & 0.09 \\     
La II & 1   & $-$2.03 & 0.00      & $-$3.13 & 0.06      & $-$0.45 & 0.07 \\     
Eu II & 1   & $-$2.51 & 0.00      & $-$3.03 & 0.06      & $-$0.35 & 0.10 \\     
C$-$H & 2   & 5.27    & 0.01      & $-$3.16 & 0.27      & $-$0.47 & 0.16 \\     
C$-$N & 1   & 5.77    & 0.00      & $-$2.07 & 0.33      & 0.63    & 0.20 \\     
Dy II & 1   & $-$1.03 & $\nodata$ & $-$2.13 & $\nodata$ & 0.55    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr462} \\ \hline
Na I  & 2   & 3.50    & 0.01 & $-$2.75 & 0.23 & 0.08    & 0.11 \\
Mg I  & 5   & 5.25    & 0.18 & $-$2.36 & 0.16 & 0.47    & 0.10 \\
Al I  & 2   & 3.16    & 0.06 & $-$3.29 & 0.35 & $-$0.47 & 0.23 \\
Si I  & 2   & 5.23    & 0.01 & $-$2.29 & 0.21 & 0.54    & 0.07 \\
Ca I  & 16  & 3.84    & 0.21 & $-$2.50 & 0.13 & 0.33    & 0.07 \\
Sc II & 8   & 0.25    & 0.13 & $-$2.91 & 0.10 & $-$0.14 & 0.08 \\
Ti I  & 15  & 2.23    & 0.14 & $-$2.73 & 0.19 & 0.10    & 0.06 \\
Ti II & 27  & 2.42    & 0.12 & $-$2.53 & 0.11 & 0.23    & 0.09 \\
V I   & 2   & 0.99    & 0.01 & $-$2.94 & 0.12 & $-$0.11 & 0.10 \\
V II  & 2   & 1.18    & 0.03 & $-$2.75 & 0.08 & 0.02    & 0.09 \\
Cr I  & 9   & 2.64    & 0.18 & $-$3.00 & 0.19 & $-$0.18 & 0.07 \\
Cr II & 1   & 2.75    & 0.00 & $-$2.89 & 0.07 & $-$0.13 & 0.07 \\
Mn I  & 6   & 2.23    & 0.08 & $-$3.21 & 0.11 & $-$0.38 & 0.08 \\
Fe I  & 164 & 4.67    & 0.21 & $-$2.83 & 0.16 & 0.00    & 0.00 \\
Fe II & 14  & 4.73    & 0.22 & $-$2.77 & 0.10 & 0.00    & 0.00 \\
Co I  & 4   & 2.33    & 0.17 & $-$2.66 & 0.17 & 0.17    & 0.10 \\
Ni I  & 7   & 3.53    & 0.17 & $-$2.69 & 0.17 & 0.14    & 0.07 \\
Zn I  & 1   & 2.06    & 0.00 & $-$2.50 & 0.05 & 0.32    & 0.13 \\
Sr II & 2   & 0.35    & 0.02 & $-$2.52 & 0.23 & 0.25    & 0.19 \\
Y II  & 3   & $-$0.45 & 0.03 & $-$2.66 & 0.09 & 0.11    & 0.09 \\
Zr II & 1   & 0.17    & 0.00 & $-$2.41 & 0.08 & 0.36    & 0.07 \\
Ba II & 5   & $-$0.55 & 0.02 & $-$2.73 & 0.14 & 0.04    & 0.10 \\
La II & 4   & $-$1.32 & 0.14 & $-$2.42 & 0.11 & 0.35    & 0.12 \\
Eu II & 2   & $-$1.68 & 0.09 & $-$2.20 & 0.12 & 0.57    & 0.13 \\
Dy II & 2   & $-$0.91 & 0.12 & $-$2.01 & 0.12 & 0.75    & 0.12 \\
C$-$H & 2   & 5.43    & 0.00 & $-$3.00 & 0.30 & $-$0.17 & 0.18 \\
C$-$N & 1   & 5.78    & 0.00 & $-$2.05 & 0.37 & 0.78    & 0.24 \\
\hline \multicolumn{8}{c}{Sgr468} \\ \hline
Na I  & 2   & 3.74    & 0.02 & $-$2.50 & 0.31 & 0.07    & 0.13 \\
Mg I  & 5   & 5.40    & 0.17 & $-$2.20 & 0.18 & 0.37    & 0.09 \\
Al I  & 2   & 2.86    & 0.40 & $-$3.59 & 0.46 & $-$1.02 & 0.33 \\
Si I  & 2   & 5.31    & 0.16 & $-$2.20 & 0.26 & 0.37    & 0.12 \\
Ca I  & 21  & 4.11    & 0.16 & $-$2.24 & 0.14 & 0.33    & 0.07 \\
Sc II & 8   & 0.54    & 0.12 & $-$2.61 & 0.12 & $-$0.02 & 0.07 \\
Ti I  & 19  & 2.37    & 0.14 & $-$2.58 & 0.22 & $-$0.01 & 0.05 \\
Ti II & 28  & 2.55    & 0.18 & $-$2.40 & 0.13 & 0.19    & 0.08 \\
V I   & 2   & 1.11    & 0.01 & $-$2.82 & 0.13 & $-$0.26 & 0.11 \\
V II  & 2   & 1.28    & 0.00 & $-$2.65 & 0.09 & $-$0.05 & 0.09 \\
Cr I  & 10  & 2.74    & 0.11 & $-$2.90 & 0.22 & $-$0.33 & 0.05 \\
Cr II & 3   & 2.94    & 0.09 & $-$2.70 & 0.09 & $-$0.11 & 0.09 \\
Mn I  & 6   & 2.27    & 0.10 & $-$3.16 & 0.13 & $-$0.60 & 0.10 \\
Fe I  & 189 & 4.93    & 0.21 & $-$2.57 & 0.20 & 0.00    & 0.00 \\
Fe II & 15  & 4.91    & 0.17 & $-$2.60 & 0.10 & 0.00    & 0.00 \\
Co I  & 4   & 2.44    & 0.29 & $-$2.55 & 0.22 & 0.02    & 0.15 \\
Ni I  & 9   & 3.49    & 0.16 & $-$2.74 & 0.18 & $-$0.17 & 0.06 \\
Zn I  & 1   & 1.73    & 0.00 & $-$2.83 & 0.05 & $-$0.27 & 0.18 \\
Sr II & 2   & 0.01    & 0.15 & $-$2.86 & 0.28 & $-$0.27 & 0.23 \\
Y II  & 3   & $-$0.97 & 0.09 & $-$3.18 & 0.10 & $-$0.58 & 0.11 \\
Zr II & 1   & $-$0.08 & 0.00 & $-$2.66 & 0.08 & $-$0.07 & 0.08 \\
Ba II & 5   & $-$0.69 & 0.11 & $-$2.87 & 0.14 & $-$0.28 & 0.09 \\
La II & 4   & $-$1.52 & 0.08 & $-$2.62 & 0.09 & $-$0.02 & 0.10 \\
Eu II & 2   & $-$1.72 & 0.00 & $-$2.24 & 0.09 & 0.35    & 0.10 \\
Dy II & 2   & $-$1.07 & 0.11 & $-$2.17 & 0.12 & 0.43    & 0.10 \\
C$-$H & 2   & 5.34    & 0.04 & $-$3.09 & 0.26 & $-$0.53 & 0.16 \\
C$-$N & 1   & 5.71    & 0.00 & $-$2.12 & 0.28 & 0.44    & 0.18 \\
\hline \multicolumn{8}{c}{Sgr476} \\ \hline
Na I  & 2   & 3.67    & 0.01      & $-$2.57 & 0.32      & 0.31    & 0.11 \\     
Mg I  & 4   & 5.19    & 0.18      & $-$2.41 & 0.20      & 0.48    & 0.10 \\     
Al I  & 2   & 2.95    & 0.32      & $-$3.50 & 0.48      & $-$0.62 & 0.33 \\     
Si I  & 2   & 4.99    & 0.26      & $-$2.52 & 0.21      & 0.36    & 0.26 \\     
Ca I  & 19  & 3.89    & 0.17      & $-$2.45 & 0.13      & 0.43    & 0.11 \\     
Sc II & 8   & 0.26    & 0.20      & $-$2.89 & 0.17      & $-$0.00 & 0.12 \\     
Ti I  & 19  & 2.12    & 0.21      & $-$2.83 & 0.23      & 0.06    & 0.07 \\     
Ti II & 28  & 2.26    & 0.24      & $-$2.69 & 0.15      & 0.20    & 0.10 \\     
V I   & 2   & 0.64    & 0.01      & $-$3.29 & 0.13      & $-$0.41 & 0.13 \\     
V II  & 2   & 0.77    & 0.10      & $-$3.16 & 0.14      & $-$0.27 & 0.13 \\     
Cr I  & 10  & 2.65    & 0.32      & $-$2.99 & 0.24      & $-$0.11 & 0.11 \\     
Cr II & 2   & 2.91    & 0.24      & $-$2.73 & 0.20      & 0.16    & 0.18 \\     
Mn I  & 6   & 2.11    & 0.06      & $-$3.32 & 0.13      & $-$0.43 & 0.13 \\     
Fe I  & 162 & 4.62    & 0.23      & $-$2.88 & 0.22      & 0.00    & 0.00 \\     
Fe II & 15  & 4.61    & 0.23      & $-$2.89 & 0.13      & 0.00    & 0.00 \\     
Co I  & 4   & 2.09    & 0.29      & $-$2.90 & 0.22      & $-$0.02 & 0.16 \\     
Ni I  & 6   & 3.31    & 0.15      & $-$2.91 & 0.18      & $-$0.03 & 0.09 \\     
Zn I  & 1   & 1.90    & 0.00      & $-$2.66 & 0.07      & 0.23    & 0.20 \\     
Sr II & 2   & 0.51    & 0.11      & $-$2.36 & 0.16      & 0.53    & 0.15 \\     
Y II  & 3   & $-$0.70 & 0.10      & $-$2.91 & 0.12      & $-$0.02 & 0.11 \\     
Zr II & 1   & $-$0.26 & 0.00      & $-$2.84 & 0.11      & 0.05    & 0.10 \\     
Ba II & 5   & $-$1.42 & 0.13      & $-$3.60 & 0.14      & $-$0.71 & 0.12 \\     
C$-$H & 2   & 5.17    & 0.01      & $-$3.26 & 0.30      & $-$0.37 & 0.19 \\     
C$-$N & 1   & 5.84    & 0.00      & $-$2.00 & 0.42      & 0.89    & 0.28 \\     
La II & 2   & $-$1.88 & $\nodata$ & $-$2.98 & $\nodata$ & $-$0.09 & $\nodata$ \\
Eu II & 3   & $-$2.71 & $\nodata$ & $-$3.23 & $\nodata$ & $-$0.34 & $\nodata$ \\
Dy II & 2   & $-$1.96 & $\nodata$ & $-$3.06 & $\nodata$ & $-$0.17 & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr488} \\ \hline
Na I  & 2   & 4.19    & 0.02      & $-$2.05 & 0.29      & 0.97    & 0.12 \\     
Mg I  & 5   & 4.84    & 0.12      & $-$2.76 & 0.16      & 0.26    & 0.08 \\     
Al I  & 2   & 3.35    & 0.10      & $-$3.10 & 0.28      & $-$0.08 & 0.16 \\     
Si I  & 2   & 4.98    & 0.04      & $-$2.53 & 0.22      & 0.49    & 0.05 \\     
Ca I  & 15  & 3.65    & 0.24      & $-$2.69 & 0.14      & 0.33    & 0.10 \\     
Sc II & 8   & 0.26    & 0.15      & $-$2.89 & 0.11      & 0.22    & 0.08 \\     
Ti I  & 12  & 2.10    & 0.20      & $-$2.85 & 0.21      & 0.17    & 0.09 \\     
Ti II & 25  & 2.25    & 0.15      & $-$2.70 & 0.12      & 0.40    & 0.09 \\     
V I   & 2   & 0.55    & 0.04      & $-$3.38 & 0.16      & $-$0.36 & 0.14 \\     
V II  & 2   & 0.92    & 0.02      & $-$3.01 & 0.15      & 0.09    & 0.12 \\     
Cr I  & 6   & 2.24    & 0.24      & $-$3.40 & 0.23      & $-$0.38 & 0.10 \\     
Mn I  & 5   & 2.02    & 0.22      & $-$3.41 & 0.15      & $-$0.39 & 0.15 \\     
Fe I  & 144 & 4.48    & 0.28      & $-$3.02 & 0.20      & 0.00    & 0.00 \\     
Fe II & 14  & 4.40    & 0.15      & $-$3.11 & 0.08      & 0.00    & 0.00 \\     
Co I  & 2   & 1.80    & 0.10      & $-$3.19 & 0.21      & $-$0.17 & 0.08 \\     
Ni I  & 7   & 3.27    & 0.24      & $-$2.95 & 0.17      & 0.07    & 0.12 \\     
Zn I  & 1   & 1.60    & 0.00      & $-$2.96 & 0.05      & 0.06    & 0.16 \\     
Sr II & 2   & $-$0.45 & 0.10      & $-$3.32 & 0.32      & $-$0.22 & 0.29 \\     
Y II  & 2   & $-$1.18 & 0.00      & $-$3.39 & 0.07      & $-$0.28 & 0.08 \\     
Ba II & 5   & $-$1.81 & 0.22      & $-$3.99 & 0.12      & $-$0.88 & 0.12 \\     
C$-$H & 2   & 4.75    & 0.07      & $-$3.68 & 0.26      & $-$0.66 & 0.17 \\     
C$-$N & 1   & 5.86    & 0.00      & $-$1.97 & 0.39      & 1.05    & 0.28 \\     
Zr II & 1   & $-$0.34 & $\nodata$ & $-$2.92 & $\nodata$ & 0.19    & $\nodata$ \\
La II & 1   & $-$1.70 & $\nodata$ & $-$2.80 & $\nodata$ & 0.31    & $\nodata$ \\
Eu II & 3   & $-$2.68 & $\nodata$ & $-$3.20 & $\nodata$ & $-$0.10 & $\nodata$ \\
Dy II & 2   & $-$1.52 & $\nodata$ & $-$2.62 & $\nodata$ & 0.49    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr492} \\ \hline
Na I  & 2  & 3.41    & 0.08      & $-$2.83 & 0.38      & $-$0.02 & 0.18 \\     
Mg I  & 3  & 4.97    & 0.16      & $-$2.63 & 0.29      & 0.17    & 0.12 \\     
Si I  & 1  & 5.07    & 0.00      & $-$2.44 & 0.21      & 0.37    & 0.07 \\     
Ca I  & 6  & 4.01    & 0.24      & $-$2.33 & 0.21      & 0.48    & 0.13 \\     
Sc II & 7  & 0.48    & 0.40      & $-$2.67 & 0.26      & $-$0.04 & 0.23 \\     
Ti I  & 2  & 2.45    & 0.29      & $-$2.50 & 0.31      & 0.30    & 0.23 \\     
Ti II & 13 & 2.33    & 0.42      & $-$2.62 & 0.24      & 0.01    & 0.21 \\     
V II  & 1  & 1.94    & 0.00      & $-$1.99 & 0.37      & 0.64    & 0.28 \\     
Cr I  & 2  & 2.29    & 0.19      & $-$3.36 & 0.38      & $-$0.55 & 0.19 \\     
Fe I  & 91 & 4.69    & 0.54      & $-$2.81 & 0.25      & 0.00    & 0.00 \\     
Fe II & 7  & 4.87    & 0.42      & $-$2.63 & 0.22      & 0.00    & 0.00 \\     
Ni I  & 1  & 3.55    & 0.00      & $-$2.67 & 0.19      & 0.14    & 0.14 \\     
Zn I  & 1  & 2.09    & 0.00      & $-$2.47 & 0.07      & 0.34    & 0.21 \\     
Sr II & 1  & $-$0.51 & 0.00      & $-$3.38 & 0.46      & $-$0.75 & 0.36 \\     
Ba II & 5  & $-$1.66 & 0.26      & $-$3.84 & 0.15      & $-$1.21 & 0.22 \\     
C$-$H & 2  & 4.98    & 0.10      & $-$3.46 & 0.29      & $-$0.65 & 0.28 \\     
Y II  & 1  & $-$0.10 & $\nodata$ & $-$2.31 & $\nodata$ & 0.32    & $\nodata$ \\
Zr II & 1  & 0.11    & $\nodata$ & $-$2.47 & $\nodata$ & 0.16    & $\nodata$ \\
La II & 1  & $-$1.32 & $\nodata$ & $-$2.42 & $\nodata$ & 0.21    & $\nodata$ \\
Eu II & 3  & $-$2.29 & $\nodata$ & $-$2.81 & $\nodata$ & $-$0.18 & $\nodata$ \\
Dy II & 2  & $-$1.52 & $\nodata$ & $-$2.62 & $\nodata$ & 0.01    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr431} \\ \hline
Na I  & 1   & 3.39    & 0.00      & $-$2.86 & 0.24      & $-$0.03 & 0.11 \\     
Mg I  & 3   & 4.69    & 0.26      & $-$2.91 & 0.24      & $-$0.08 & 0.16 \\     
Al I  & 2   & 2.53    & 0.06      & $-$3.92 & 0.32      & $-$1.09 & 0.15 \\     
Si I  & 2   & 5.31    & 0.01      & $-$2.20 & 0.23      & 0.63    & 0.14 \\     
Ca I  & 10  & 3.57    & 0.19      & $-$2.77 & 0.13      & 0.05    & 0.11 \\     
Sc II & 6   & 0.18    & 0.11      & $-$2.97 & 0.11      & $-$0.11 & 0.10 \\     
Ti I  & 7   & 2.23    & 0.16      & $-$2.72 & 0.19      & 0.10    & 0.09 \\     
Ti II & 23  & 2.27    & 0.27      & $-$2.68 & 0.15      & 0.19    & 0.12 \\     
V I   & 2   & 0.98    & 0.03      & $-$2.95 & 0.10      & $-$0.13 & 0.15 \\     
Cr I  & 5   & 2.49    & 0.30      & $-$3.15 & 0.26      & $-$0.33 & 0.14 \\     
Cr II & 1   & 2.70    & 0.00      & $-$2.94 & 0.08      & $-$0.08 & 0.10 \\     
Mn I  & 4   & 2.30    & 0.13      & $-$3.14 & 0.13      & $-$0.31 & 0.12 \\     
Fe I  & 133 & 4.68    & 0.34      & $-$2.82 & 0.18      & 0.00    & 0.00 \\     
Fe II & 14  & 4.64    & 0.31      & $-$2.87 & 0.13      & 0.00    & 0.00 \\     
Co I  & 4   & 2.41    & 0.22      & $-$2.58 & 0.18      & 0.24    & 0.12 \\     
Ni I  & 4   & 3.53    & 0.21      & $-$2.69 & 0.19      & 0.13    & 0.12 \\     
Zn I  & 1   & 2.22    & 0.00      & $-$2.34 & 0.07      & 0.48    & 0.13 \\     
Sr II & 2   & 1.04    & 0.01      & $-$1.83 & 0.14      & 1.03    & 0.14 \\     
Y II  & 3   & $-$0.53 & 0.06      & $-$2.74 & 0.11      & 0.13    & 0.11 \\     
Ba II & 5   & $-$0.84 & 0.10      & $-$3.02 & 0.16      & $-$0.16 & 0.12 \\     
La II & 3   & $-$1.38 & 0.04      & $-$2.48 & 0.11      & 0.39    & 0.12 \\     
Eu II & 2   & $-$1.87 & 0.09      & $-$2.39 & 0.15      & 0.47    & 0.15 \\     
C$-$H & 2   & 5.50    & 0.02      & $-$2.93 & 0.30      & $-$0.11 & 0.20 \\     
C$-$N & 1   & 4.98    & 0.00      & $-$2.85 & 0.89      & $-$0.03 & 1.05 \\     
Zr II & 1   & 0.07    & $\nodata$ & $-$2.52 & $\nodata$ & 0.35    & $\nodata$ \\
Dy II & 2   & $-$0.93 & $\nodata$ & $-$2.03 & $\nodata$ & 0.84    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr434} \\ \hline
Na I  & 2   & 4.48    & 0.02      & $-$1.76 & 0.23      & 0.94    & 0.09 \\     
Mg I  & 5   & 5.12    & 0.13      & $-$2.48 & 0.14      & 0.22    & 0.08 \\     
Al I  & 2   & 3.21    & 0.18      & $-$3.24 & 0.40      & $-$0.54 & 0.27 \\     
Si I  & 2   & 5.56    & 0.12      & $-$1.95 & 0.21      & 0.76    & 0.10 \\     
Ca I  & 13  & 4.08    & 0.19      & $-$2.26 & 0.12      & 0.45    & 0.08 \\     
Sc II & 7   & 0.49    & 0.11      & $-$2.66 & 0.10      & $-$0.02 & 0.08 \\     
Ti I  & 11  & 2.41    & 0.13      & $-$2.54 & 0.17      & 0.16    & 0.06 \\     
Ti II & 23  & 2.57    & 0.21      & $-$2.38 & 0.14      & 0.27    & 0.10 \\     
V I   & 2   & 1.38    & 0.10      & $-$2.56 & 0.19      & 0.15    & 0.13 \\     
V II  & 2   & 1.19    & 0.25      & $-$2.74 & 0.20      & $-$0.09 & 0.23 \\     
Cr I  & 4   & 2.61    & 0.08      & $-$3.03 & 0.18      & $-$0.33 & 0.05 \\     
Cr II & 1   & 3.19    & 0.00      & $-$2.45 & 0.07      & 0.20    & 0.08 \\     
Mn I  & 5   & 2.18    & 0.17      & $-$3.25 & 0.12      & $-$0.55 & 0.12 \\     
Fe I  & 137 & 4.80    & 0.24      & $-$2.70 & 0.16      & 0.00    & 0.00 \\     
Fe II & 14  & 4.85    & 0.25      & $-$2.65 & 0.11      & 0.00    & 0.00 \\     
Co I  & 4   & 2.62    & 0.07      & $-$2.37 & 0.14      & 0.33    & 0.05 \\     
Ni I  & 2   & 3.68    & 0.01      & $-$2.54 & 0.15      & 0.16    & 0.03 \\     
Zn I  & 1   & 1.99    & 0.00      & $-$2.57 & 0.05      & 0.13    & 0.12 \\     
Sr II & 2   & 0.57    & 0.08      & $-$2.30 & 0.22      & 0.35    & 0.18 \\     
Y II  & 2   & $-$0.54 & 0.00      & $-$2.75 & 0.07      & $-$0.11 & 0.10 \\     
Zr II & 1   & 0.21    & 0.00      & $-$2.37 & 0.08      & 0.28    & 0.09 \\     
Ba II & 5   & $-$1.04 & 0.08      & $-$3.22 & 0.10      & $-$0.57 & 0.10 \\     
C$-$H & 2   & 5.78    & 0.02      & $-$2.66 & 0.27      & 0.05    & 0.18 \\     
C$-$N & 1   & 5.93    & 0.00      & $-$1.90 & 0.32      & 0.81    & 0.22 \\     
Eu II & 3   & $-$2.07 & $\nodata$ & $-$2.59 & $\nodata$ & 0.06    & $\nodata$ \\
Dy II & 2   & $-$1.44 & $\nodata$ & $-$2.54 & $\nodata$ & 0.11    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr453} \\ \hline
Na I  & 2   & 3.96    & 0.01      & $-$2.28 & 0.33      & $-$0.03 & 0.11 \\     
Mg I  & 3   & 5.71    & 0.13      & $-$1.90 & 0.21      & 0.36    & 0.12 \\     
Si I  & 1   & 5.34    & 0.00      & $-$2.18 & 0.21      & 0.08    & 0.05 \\     
Ca I  & 23  & 4.51    & 0.20      & $-$1.83 & 0.18      & 0.42    & 0.07 \\     
Sc II & 6   & 1.02    & 0.25      & $-$2.13 & 0.15      & $-$0.10 & 0.13 \\     
Ti I  & 16  & 2.80    & 0.26      & $-$2.15 & 0.34      & 0.10    & 0.14 \\     
Ti II & 25  & 3.21    & 0.33      & $-$1.74 & 0.20      & 0.28    & 0.14 \\     
V I   & 2   & 1.18    & 0.14      & $-$2.75 & 0.26      & $-$0.50 & 0.16 \\     
Cr I  & 9   & 3.25    & 0.21      & $-$2.39 & 0.31      & $-$0.14 & 0.11 \\     
Cr II & 1   & 3.30    & 0.00      & $-$2.34 & 0.12      & $-$0.32 & 0.10 \\     
Mn I  & 6   & 2.69    & 0.09      & $-$2.74 & 0.14      & $-$0.49 & 0.13 \\     
Fe I  & 152 & 5.25    & 0.23      & $-$2.25 & 0.23      & 0.00    & 0.00 \\     
Fe II & 13  & 5.48    & 0.24      & $-$2.02 & 0.18      & 0.00    & 0.00 \\     
Co I  & 3   & 3.11    & 0.12      & $-$1.88 & 0.25      & 0.37    & 0.12 \\     
Ni I  & 10  & 4.02    & 0.16      & $-$2.20 & 0.18      & 0.05    & 0.08 \\     
Zn I  & 1   & 2.37    & 0.00      & $-$2.19 & 0.09      & 0.06    & 0.28 \\     
Sr II & 2   & 0.27    & 0.28      & $-$2.60 & 0.27      & $-$0.58 & 0.25 \\     
Y II  & 3   & $-$0.28 & 0.10      & $-$2.49 & 0.12      & $-$0.47 & 0.12 \\     
Zr II & 1   & 0.18    & 0.00      & $-$2.40 & 0.12      & $-$0.38 & 0.14 \\     
Ba II & 5   & $-$0.06 & 0.11      & $-$2.24 & 0.19      & $-$0.22 & 0.13 \\     
La II & 3   & $-$1.14 & 0.14      & $-$2.24 & 0.12      & $-$0.22 & 0.18 \\     
Eu II & 2   & $-$1.32 & 0.11      & $-$1.84 & 0.10      & 0.18    & 0.19 \\     
Dy II & 2   & $-$0.13 & 0.01      & $-$1.23 & 0.09      & 0.79    & 0.11 \\     
C$-$H & 2   & 5.58    & 0.00      & $-$2.85 & 0.22      & $-$0.60 & 0.24 \\     
C$-$N & 1   & 6.09    & 0.00      & $-$1.74 & 0.28      & 0.51    & 0.24 \\     
Al I  & 1   & 3.93    & $\nodata$ & $-$2.52 & $\nodata$ & $-$0.26 & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr459} \\ \hline
Na I  & 2   & 3.58    & 0.00      & $-$2.66 & 0.34      & 0.00    & 0.14 \\     
Mg I  & 3   & 5.36    & 0.09      & $-$2.24 & 0.21      & 0.43    & 0.07 \\     
Al I  & 2   & 2.97    & 0.22      & $-$3.49 & 0.37      & $-$0.83 & 0.20 \\     
Si I  & 2   & 5.01    & 0.28      & $-$2.50 & 0.28      & 0.16    & 0.20 \\     
Ca I  & 21  & 4.08    & 0.22      & $-$2.26 & 0.14      & 0.40    & 0.09 \\     
Sc II & 7   & 0.40    & 0.14      & $-$2.75 & 0.13      & $-$0.22 & 0.09 \\     
Ti I  & 17  & 2.45    & 0.22      & $-$2.50 & 0.27      & 0.16    & 0.09 \\     
Ti II & 30  & 2.77    & 0.26      & $-$2.18 & 0.17      & 0.34    & 0.11 \\     
V I   & 2   & 0.95    & 0.10      & $-$2.98 & 0.19      & $-$0.32 & 0.12 \\     
V II  & 2   & 1.59    & 0.27      & $-$2.34 & 0.25      & 0.19    & 0.22 \\     
Cr I  & 10  & 2.66    & 0.19      & $-$2.98 & 0.27      & $-$0.32 & 0.09 \\     
Cr II & 2   & 3.04    & 0.22      & $-$2.61 & 0.18      & $-$0.08 & 0.18 \\     
Mn I  & 6   & 2.32    & 0.09      & $-$3.11 & 0.13      & $-$0.45 & 0.12 \\     
Fe I  & 168 & 4.84    & 0.22      & $-$2.66 & 0.21      & 0.00    & 0.00 \\     
Fe II & 16  & 4.98    & 0.26      & $-$2.53 & 0.14      & 0.00    & 0.00 \\     
Co I  & 3   & 2.48    & 0.08      & $-$2.51 & 0.22      & 0.15    & 0.06 \\     
Ni I  & 9   & 3.60    & 0.15      & $-$2.62 & 0.17      & 0.04    & 0.08 \\     
Zn I  & 1   & 2.25    & 0.00      & $-$2.32 & 0.06      & 0.35    & 0.20 \\     
Sr II & 2   & 0.01    & 0.07      & $-$2.86 & 0.19      & $-$0.34 & 0.13 \\     
Y II  & 3   & $-$0.97 & 0.06      & $-$3.18 & 0.10      & $-$0.65 & 0.12 \\     
Zr II & 1   & $-$0.27 & 0.00      & $-$2.85 & 0.10      & $-$0.33 & 0.10 \\     
Ba II & 5   & $-$1.17 & 0.10      & $-$3.35 & 0.13      & $-$0.82 & 0.11 \\     
Eu II & 2   & $-$2.45 & 0.09      & $-$2.97 & 0.12      & $-$0.45 & 0.15 \\     
C$-$H & 2   & 5.06    & 0.01      & $-$3.37 & 0.25      & $-$0.71 & 0.17 \\     
C$-$N & 1   & 5.73    & 0.00      & $-$2.10 & 0.30      & 0.56    & 0.20 \\     
La II & 2   & $-$1.64 & $\nodata$ & $-$2.74 & $\nodata$ & $-$0.21 & $\nodata$ \\
Dy II & 2   & $-$1.51 & $\nodata$ & $-$2.61 & $\nodata$ & $-$0.09 & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr471} \\ \hline
Na I  & 2   & 3.37    & 0.00      & $-$2.87 & 0.25      & 0.28    & 0.12 \\     
Mg I  & 4   & 4.79    & 0.10      & $-$2.81 & 0.16      & 0.33    & 0.06 \\     
Al I  & 2   & 2.71    & 0.10      & $-$3.74 & 0.18      & $-$0.60 & 0.08 \\     
Si I  & 2   & 4.88    & 0.08      & $-$2.63 & 0.21      & 0.51    & 0.09 \\     
Ca I  & 13  & 3.36    & 0.21      & $-$2.98 & 0.13      & 0.16    & 0.08 \\     
Sc II & 8   & 0.05    & 0.17      & $-$3.10 & 0.11      & 0.04    & 0.07 \\     
Ti I  & 8   & 1.91    & 0.15      & $-$3.04 & 0.19      & 0.10    & 0.07 \\     
Ti II & 24  & 2.08    & 0.15      & $-$2.87 & 0.11      & 0.27    & 0.08 \\     
V I   & 3   & 0.84    & 0.18      & $-$3.09 & 0.19      & 0.05    & 0.13 \\     
Cr I  & 5   & 2.02    & 0.27      & $-$3.62 & 0.22      & $-$0.47 & 0.12 \\     
Mn I  & 5   & 1.76    & 0.13      & $-$3.67 & 0.12      & $-$0.53 & 0.10 \\     
Fe I  & 121 & 4.36    & 0.24      & $-$3.14 & 0.17      & 0.00    & 0.00 \\     
Fe II & 12  & 4.36    & 0.09      & $-$3.14 & 0.08      & 0.00    & 0.00 \\     
Co I  & 4   & 2.00    & 0.24      & $-$2.99 & 0.20      & 0.15    & 0.13 \\     
Ni I  & 3   & 3.17    & 0.05      & $-$3.05 & 0.20      & 0.10    & 0.07 \\     
Sr II & 2   & $-$1.64 & 0.24      & $-$4.51 & 0.24      & $-$1.37 & 0.22 \\     
Ba II & 5   & $-$1.51 & 0.19      & $-$3.69 & 0.12      & $-$0.55 & 0.11 \\     
C$-$H & 2   & 4.77    & 0.11      & $-$3.66 & 0.28      & $-$0.52 & 0.18 \\     
Zn I  & 1   & 1.62    & $\nodata$ & $-$2.94 & $\nodata$ & 0.21    & $\nodata$ \\
Y II  & 1   & $-$1.11 & $\nodata$ & $-$3.32 & $\nodata$ & $-$0.18 & $\nodata$ \\
Zr II & 1   & $-$0.47 & $\nodata$ & $-$3.05 & $\nodata$ & 0.09    & $\nodata$ \\
La II & 3   & $-$1.74 & $\nodata$ & $-$2.84 & $\nodata$ & 0.30    & $\nodata$ \\
Eu II & 2   & $-$2.26 & $\nodata$ & $-$2.78 & $\nodata$ & 0.36    & $\nodata$ \\
Dy II & 2   & $-$1.38 & $\nodata$ & $-$2.48 & $\nodata$ & 0.66    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr505} \\ \hline
Na I  & 2   & 3.42    & 0.02      & $-$2.82 & 0.25      & 0.24    & 0.12 \\     
Mg I  & 4   & 4.95    & 0.18      & $-$2.65 & 0.17      & 0.41    & 0.10 \\     
Al I  & 2   & 3.27    & 0.12      & $-$3.18 & 0.24      & $-$0.12 & 0.15 \\     
Si I  & 1   & 5.19    & 0.00      & $-$2.33 & 0.21      & 0.74    & 0.07 \\     
Ca I  & 12  & 3.41    & 0.15      & $-$2.93 & 0.12      & 0.13    & 0.08 \\     
Sc II & 8   & 0.06    & 0.19      & $-$3.09 & 0.11      & $-$0.01 & 0.08 \\     
Ti I  & 8   & 1.83    & 0.19      & $-$3.12 & 0.19      & $-$0.06 & 0.09 \\     
Ti II & 22  & 2.16    & 0.20      & $-$2.80 & 0.13      & 0.29    & 0.10 \\     
V I   & 2   & 0.63    & 0.10      & $-$3.30 & 0.16      & $-$0.24 & 0.15 \\     
V II  & 2   & 1.05    & 0.02      & $-$2.88 & 0.07      & 0.20    & 0.07 \\     
Cr I  & 5   & 2.00    & 0.22      & $-$3.64 & 0.21      & $-$0.58 & 0.10 \\     
Mn I  & 6   & 1.94    & 0.21      & $-$3.49 & 0.13      & $-$0.43 & 0.13 \\     
Fe I  & 140 & 4.44    & 0.29      & $-$3.06 & 0.17      & 0.00    & 0.00 \\     
Fe II & 14  & 4.41    & 0.17      & $-$3.09 & 0.08      & 0.00    & 0.00 \\     
Co I  & 4   & 1.73    & 0.17      & $-$3.26 & 0.17      & $-$0.19 & 0.13 \\     
Ni I  & 4   & 3.11    & 0.18      & $-$3.11 & 0.20      & $-$0.05 & 0.09 \\     
Zn I  & 1   & 1.87    & 0.00      & $-$2.69 & 0.06      & 0.37    & 0.13 \\     
Sr II & 2   & $-$0.35 & 0.24      & $-$3.22 & 0.37      & $-$0.13 & 0.34 \\     
Y II  & 2   & $-$1.45 & 0.06      & $-$3.66 & 0.10      & $-$0.58 & 0.09 \\     
Zr II & 1   & $-$0.37 & 0.00      & $-$2.95 & 0.07      & 0.13    & 0.07 \\     
Ba II & 5   & $-$1.80 & 0.27      & $-$3.98 & 0.15      & $-$0.89 & 0.15 \\     
C$-$H & 2   & 4.76    & 0.04      & $-$3.67 & 0.31      & $-$0.61 & 0.22 \\     
La II & 2   & $-$1.55 & $\nodata$ & $-$2.65 & $\nodata$ & 0.44    & $\nodata$ \\
Eu II & 3   & $-$2.50 & $\nodata$ & $-$3.02 & $\nodata$ & 0.07    & $\nodata$ \\
Dy II & 2   & $-$1.63 & $\nodata$ & $-$2.73 & $\nodata$ & 0.36    & $\nodata$ \\
\hline \multicolumn{8}{c}{Sgr504} \\ \hline
Na I  & 2   & 3.63    & 0.11      & $-$2.61 & 0.31      & 0.06    & 0.15 \\     
Mg I  & 4   & 5.13    & 0.09      & $-$2.47 & 0.18      & 0.20    & 0.06 \\     
Al I  & 2   & 3.45    & 0.01      & $-$3.00 & 0.36      & $-$0.33 & 0.20 \\     
Si I  & 2   & 5.33    & 0.28      & $-$2.18 & 0.32      & 0.49    & 0.21 \\     
Ca I  & 17  & 4.03    & 0.16      & $-$2.31 & 0.13      & 0.36    & 0.08 \\     
Sc II & 8   & 0.42    & 0.16      & $-$2.73 & 0.12      & 0.01    & 0.08 \\     
Ti I  & 15  & 2.24    & 0.12      & $-$2.71 & 0.21      & $-$0.05 & 0.06 \\     
Ti II & 26  & 2.43    & 0.14      & $-$2.53 & 0.13      & 0.22    & 0.08 \\     
V I   & 2   & 0.87    & 0.08      & $-$3.06 & 0.13      & $-$0.39 & 0.15 \\     
V II  & 2   & 1.07    & 0.11      & $-$2.86 & 0.13      & $-$0.12 & 0.13 \\     
Cr I  & 9   & 2.68    & 0.27      & $-$2.96 & 0.22      & $-$0.29 & 0.10 \\     
Cr II & 2   & 3.02    & 0.09      & $-$2.62 & 0.10      & 0.13    & 0.10 \\     
Mn I  & 5   & 2.22    & 0.09      & $-$3.21 & 0.12      & $-$0.54 & 0.11 \\     
Fe I  & 169 & 4.83    & 0.27      & $-$2.67 & 0.19      & 0.00    & 0.00 \\     
Fe II & 15  & 4.76    & 0.19      & $-$2.74 & 0.10      & 0.00    & 0.00 \\     
Co I  & 4   & 2.18    & 0.18      & $-$2.81 & 0.21      & $-$0.14 & 0.11 \\     
Ni I  & 5   & 3.57    & 0.14      & $-$2.65 & 0.23      & 0.02    & 0.08 \\     
Zn I  & 1   & 1.94    & 0.00      & $-$2.62 & 0.06      & 0.05    & 0.17 \\     
Sr II & 2   & 0.30    & 0.06      & $-$2.57 & 0.21      & 0.17    & 0.16 \\     
Y II  & 3   & $-$0.74 & 0.12      & $-$2.95 & 0.10      & $-$0.20 & 0.10 \\     
Zr II & 1   & $-$0.13 & 0.00      & $-$2.71 & 0.10      & 0.03    & 0.08 \\     
Ba II & 5   & $-$1.09 & 0.08      & $-$3.27 & 0.11      & $-$0.53 & 0.08 \\     
Eu II & 2   & $-$2.24 & 0.08      & $-$2.76 & 0.10      & $-$0.02 & 0.11 \\     
C$-$H & 2   & 5.31    & 0.01      & $-$3.12 & 0.26      & $-$0.45 & 0.16 \\     
C$-$N & 1   & 5.80    & 0.00      & $-$2.03 & 0.31      & 0.64    & 0.20 \\     
La II & 1   & $-$1.39 & $\nodata$ & $-$2.49 & $\nodata$ & 0.26    & $\nodata$ \\
Dy II & 2   & $-$1.51 & $\nodata$ & $-$2.61 & $\nodata$ & 0.13    & $\nodata$ \\
\enddata
\tablenotetext{}{}
\end{deluxetable*}


==> tab03_stub.tex <==
\begin{deluxetable}{lrrrrrrr} 
\tablecaption{Chemical Abundances for the Sgr sample with the number of lines used for each element and associated total uncertainties.}
\label{tab:abund}
\tabletypesize{\scriptsize}
\tablehead{\colhead{El.} & \colhead{N} & \colhead{$\log \epsilon (\rm{X})_{\*}$} & \colhead{$\sigma$} & \colhead{${\rm [X/H]}$} & \colhead{$\sigma_{\rm [X/H]}$} & \colhead{${\rm [X/Fe]}$} & \colhead{$\sigma_{\rm [X/Fe]}$}}
\startdata
\multicolumn{8}{c}{Sgr2} \\ 
\hline
Na I  & 2   & 3.96    & 0.07      & $-$2.28 & 0.25      & 0.38    & 0.12 \\     
Mg I  & 4   & 5.25    & 0.13      & $-$2.35 & 0.16      & 0.31    & 0.08 \\     
Al I  & 2   & 3.37    & 0.22      & $-$3.09 & 0.42      & $-$0.43 & 0.29 \\     
Si I  & 2   & 5.34    & 0.21      & $-$2.17 & 0.26      & 0.49    & 0.16 \\     
Ca I  & 15  & 3.97    & 0.16      & $-$2.37 & 0.13      & 0.29    & 0.06 \\     
Sc II & 7   & 0.52    & 0.12      & $-$2.63 & 0.10      & $-$0.08 & 0.06 \\     
Ti I  & 14  & 2.30    & 0.17      & $-$2.65 & 0.20      & 0.01    & 0.07 \\     
Ti II & 29  & 2.57    & 0.15      & $-$2.38 & 0.12      & 0.17    & 0.07 \\     
V I   & 2   & 0.95    & 0.01      & $-$2.99 & 0.12      & $-$0.33 & 0.10 \\     
V II  & 2   & 1.16    & 0.10      & $-$2.77 & 0.10      & $-$0.22 & 0.11 \\     
Cr I  & 9   & 2.80    & 0.12      & $-$2.84 & 0.19      & $-$0.19 & 0.05 \\     
Cr II & 3   & 3.07    & 0.14      & $-$2.57 & 0.11      & $-$0.02 & 0.10 \\     
Mn I  & 6   & 2.27    & 0.08      & $-$3.16 & 0.11      & $-$0.51 & 0.09 \\     
Fe I  & 154 & 4.84    & 0.20      & $-$2.66 & 0.17      & 0.00    & 0.00 \\     
Fe II & 15  & 4.95    & 0.12      & $-$2.55 & 0.10      & 0.00    & 0.00 \\     
Co I  & 4   & 2.29    & 0.21      & $-$2.70 & 0.17      & $-$0.04 & 0.12 \\     
Ni I  & 4   & 3.59    & 0.21      & $-$2.63 & 0.24      & 0.03    & 0.12 \\     
Zn I  & 1   & 2.06    & 0.00      & $-$2.50 & 0.06      & 0.16    & 0.13 \\     
Sr II & 2   & 0.61    & 0.11      & $-$2.26 & 0.18      & 0.29    & 0.15 \\     
Y II  & 3   & $-$0.59 & 0.07      & $-$2.80 & 0.10      & $-$0.25 & 0.09 \\     
Zr II & 1   & 0.14    & 0.00      & $-$2.44 & 0.10      & 0.11    & 0.06 \\     
Ba II & 5   & $-$0.94 & 0.17      & $-$3.12 & 0.13      & $-$0.57 & 0.10 \\     
La II & 3   & $-$1.94 & 0.10      & $-$3.04 & 0.10      & $-$0.49 & 0.13 \\     
C-H & 2   & 5.44    & 0.01      & $-$2.99 & 0.29      & $-$0.34 & 0.19 \\     
C-N & 1   & 6.22    & 0.00      & $-$1.61 & 0.40      & 1.05    & 0.27 \\     
Eu II & 3   & $-$2.27 & \nodata & $-$2.79 & \nodata & $-$0.23 & \nodata \\
Dy II & 1   & $-$0.60 & \nodata & $-$1.70 & \nodata & 0.86    & \nodata 
\enddata
\tablenotetext{}{}
\end{deluxetable}


==> tab04.tex <==
\begin{deluxetable}{lrrrrr}
\tablecaption{
Systematic elemental abundance uncertainties for an example star, Sgr421 (\Gaia~DR3~620763790933951488).
}
\label{tab:unc_example}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{Element} & \colhead{$\Delta_{\rm{\teff}}$} & \colhead{$\Delta_{\rm{\logg}}$} & \colhead{$\Delta_{\rm{\vt}}$} & \colhead{$\Delta_{\rm{\feh}}$} & \colhead{$\sigma_{\rm{sys.}}$} \\
\colhead{} & \colhead{$\pm 122$\,K} & \colhead{$\pm 0.2$\,dex} & \colhead{$\pm 0.3$\,\kmsec} & \colhead{$\pm 0.16$\,dex} & \colhead{}
}
\startdata
Na I & 0.15 & $-$0.05 & $-$0.16 & $-$0.04 & 0.22 \\
Mg I & 0.11 & $-$0.05 & $-$0.05 & $-$0.01 & 0.13 \\
Al I & 0.18 & $-$0.06 & $-$0.11 & $-$0.03 & 0.22 \\
Si I & 0.17 & $-$0.05 & $-$0.05 & $-$0.01 & 0.18 \\
Ca I & 0.10 & $-$0.02 & $-$0.04 & $-$0.00 & 0.11 \\
Sc II & $-$0.00 & 0.08 & $-$0.06 & 0.01 & 0.10 \\
Ti I & 0.18 & $-$0.02 & $-$0.03 & $-$0.01 & 0.18 \\
Ti II & 0.06 & 0.07 & $-$0.08 & 0.02 & 0.12 \\
V I & 0.21 & 0.02 & 0.06 & 0.05 & 0.22 \\
V II & $-$0.00 & 0.08 & 0.01 & 0.02 & 0.08 \\
Cr I & 0.16 & $-$0.02 & $-$0.02 & $-$0.01 & 0.16 \\
Cr II & $-$0.01 & 0.08 & $-$0.01 & 0.01 & 0.08 \\
Mn I & 0.09 & $-$0.04 & $-$0.01 & $-$0.01 & 0.10 \\
Fe I & 0.14 & $-$0.02 & $-$0.06 & $-$0.01 & 0.16 \\
Fe II & 0.02 & 0.08 & $-$0.03 & 0.02 & 0.09 \\
Co I & 0.14 & $-$0.03 & $-$0.03 & $-$0.01 & 0.15 \\
Ni I & 0.15 & $-$0.01 & $-$0.01 & $-$0.00 & 0.15 \\
Zn I & 0.04 & 0.03 & $-$0.01 & 0.01 & 0.06 \\
Sr II & 0.06 & 0.04 & $-$0.23 & $-$0.02 & 0.24 \\
Y II & 0.08 & 0.08 & $-$0.02 & 0.03 & 0.11 \\
Zr II & 0.04 & 0.09 & 0.01 & 0.02 & 0.10 \\
Ba II & 0.08 & 0.06 & $-$0.13 & $-$0.01 & 0.17 \\
La II & 0.07 & 0.07 & $-$0.00 & 0.03 & 0.10 \\
Eu II & 0.08 & 0.07 & 0.01 & 0.03 & 0.11 \\
Dy II & 0.02 & 0.04 & $-$0.07 & $-$0.02 & 0.08 \\
C-H & 0.28 & $-$0.07 & 0.02 & 0.06 & 0.29 \\
C-N & 0.33 & $-$0.02 & 0.06 & 0.05 & 0.34
\enddata
\end{deluxetable}


==> tab05.tex <==
\begin{deluxetable}{lrrrrrr}
\tablecaption{
The mean abundances and corresponding spreads for the Sgr stars in core vs. stream.
}
\label{tab:core_stream_comp}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{Element} & \multicolumn{2}{c}{Mean} & \multicolumn{2}{c}{Spread} & \multicolumn{2}{c}{Number} \\
\colhead{} & \colhead{Stream} & \colhead{Core} & \colhead{Stream} & \colhead{Core} & \colhead{Stream} & \colhead{Core}
}
\startdata
% v4 abund version
% $[$C/Fe$]$ & -0.37 & -0.47 & 0.32 & 0.24 & 15 & 22 \\ % pre-correction
$[$C/Fe$]$ & 0.18 & 0.24 & 0.30 & 0.22 & 15 & 22 \\
$[$Na I/Fe$]$ & 0.35 & 0.31 & 0.40 & 0.31 & 15 & 22 \\
$[$Mg I/Fe$]$ & 0.22 & 0.34 & 0.18 & 0.10 & 15 & 22 \\
$[$Al I/Fe$]$ & $-$0.59 & $-$0.44 & 0.33 & 0.29 & 14 & 21 \\
$[$Si I/Fe$]$ & 0.45 & 0.46 & 0.26 & 0.13 & 15 & 22 \\
$[$Ca I/Fe$]$ & 0.27 & 0.31 & 0.13 & 0.09 & 15 & 22 \\
$[$Sc II/Fe$]$ & 0.01 & $-$0.01 & 0.17 & 0.13 & 15 & 22 \\
$[$Ti II/Fe$]$ & 0.24 & 0.26 & 0.10 & 0.10 & 15 & 22 \\
$[$Cr I/Fe$]$ & $-$0.32 & $-$0.33 & 0.14 & 0.13 & 15 & 22 \\
% $[$Cr II/Fe$]$ & $-$0.03 & 0.01 & 0.14 & 0.12 & 11 & 12 \\
$[$Mn I/Fe$]$ & $-$0.50 & $-$0.47 & 0.13 & 0.12 & 14 & 21 \\
$[$Co I/Fe$]$ & 0.12 & 0.06 & 0.18 & 0.15 & 15 & 21 \\
$[$Ni I/Fe$]$ & 0.03 & 0.02 & 0.16 & 0.11 & 15 & 22 \\
$[$Zn I/Fe$]$ & 0.08 & 0.22 & 0.18 & 0.20 & 12 & 20 \\
$[$Sr II/Fe$]$ & $-$0.11 & $-$0.05 & 0.49 & 0.42 & 15 & 22 \\
$[$Y II/Fe$]$ & $-$0.29 & $-$0.27 & 0.30 & 0.22 & 12 & 19 \\
$[$Zr II/Fe$]$ & 0.05 & 0.14 & 0.24 & 0.18 & 9 & 16 \\
$[$Ba II/Fe$]$ & $-$0.52 & $-$0.68 & 0.48 & 0.39 & 15 & 22 \\
$[$La II/Fe$]$ & 0.06 & $-$0.12 & 0.34 & 0.32 & 8 & 6 \\
$[$Eu II/Fe$]$ & $-$0.04 & $-$0.24 & 0.43 & 0.37 & 10 & 8 \\
$[$Dy II/Fe$]$ & 0.61 & 0.48 & 0.43 & 0.21 & 6 & 4
\enddata
\end{deluxetable}



==> tab06.tex <==
\begin{deluxetable}{lrrrrl}
\tablecaption{Ba and Eu abundances of the eight \rpro-enhanced stars discussed in Section~\ref{sec:rpe_stars}.}
\label{tab:rproc_ste_par}
\tabletypesize{\scriptsize}
\tablewidth{\linewidth}
\tablehead{
    \colhead{Star Name} & \colhead{$\ce{[Fe/H]}$} & \colhead{$\ce{[Ba/Fe]}$} & \colhead{$\ce{[Eu/Fe]}$} & \colhead{$\ce{[Ba/Eu]}$} & \colhead{Classification}
    \\
    \colhead{} & \colhead{(${\rm dex}$)} & \colhead{(${\rm dex}$)} & \colhead{(${\rm dex}$)} & \colhead{(${\rm dex}$)} & \colhead{}}
\startdata
{\large\fullFillCircle} Sgr9   & $-$1.85 &    0.18 & 0.58 & $-$0.39 & r-I \\
{\large\noFillCircle} Sgr421   & $-$2.81 &    0.47 & 1.14 & $-$0.66 & r-II \\
{\large\noFillCircle} Sgr422   & $-$1.93 &    0.12 & 0.43 & $-$0.31 & r-I \\
{\large\noFillCircle} Sgr423   & $-$2.52 & $-$0.44 & 0.24 & $-$0.67 & \sim r-I \\
{\large\noFillCircle} Sgr428   & $-$2.39 &    0.06 & 0.64 & $-$0.58 & r-I, \sim r-II \\
{\large\noFillCircle} Sgr431   & $-$2.82 & $-$0.16 & 0.47 & $-$0.63 & r-I \\
{\large\fullFillCircle} Sgr462 & $-$2.83 &    0.04 & 0.57 & $-$0.53 & r-I \\
{\large\fullFillCircle} Sgr468 & $-$2.57 & $-$0.28 & 0.35 & $-$0.63 & r-I
\enddata
% \tablenotetext{}{}
\end{deluxetable}
